Monitoring Distributed Component-Based Systems

This paper addresses the online monitoring of distributed component-based systems with multi-party interactions against user-provided properties expressed in linear-temporal logic and referring to global states. We consider intrinsically independent components whose interactions are partitioned on distributed controllers. In this context, the problem that arises is that a global state of the system is not available to the monitor. Instead, we attach local controllers to schedulers to retrieve the concurrent local traces. Local traces are sent to a global observer which reconstructs the set of global traces that are compatible with the local ones, in a concurrency-preserving fashion. In this context, the reconstruction of the global traces is done on-the-fly using a lattice of partial states encoding the global traces compatible with the locally-observed traces. We implemented our monitoring approach in a prototype tool called RVDIST. RVDIST executes in parallel with the distributed model and takes as input the events generated from each scheduler and outputs the evaluated computation lattice. Our experiments show that, thanks to the optimisation applied in the online monitoring algorithm, i) the size of the constructed computation lattice is insensitive to the the number of received events, (ii) the lattice size is kept reasonable and (iii) the overhead of the monitoring process is cheap.

==> abstract-dcomp-model-old.tex <==
%
%\section{Distributed Component-based Systems with Multi-party Interactions}
%
In the following, we describe our assumptions on the distributed component-based system with multi-party interactions under scrutiny.
%
To be as general as possible, our monitoring approach assumes that the behavior of system under scrutiny can be modelled with the semantics described below.
%
However, neither the exact model nor the behavior of the system are known.
%
How the behaviors of the components and the schedulers are obtained is irrelevant.
%
Inspiring from conformance testing theory, we refer to this hypothesis as the \textbf{monitoring hypothesis}.
%
Consequently, our monitoring approach can be applied to (component-based) systems whose behavior can be modelled as described in the sequel.
%
The semantics of the following is similar to and compatible with other models for describing distributed computations (see~\ref{sec:rw} for a comparison with other models and possible translations between models).
%

%
Our concern is monitoring the behavior of a distributed system with respect to the a given property $\varphi$ which refers to the global state of the system.
%
Since actual global trace of a distributed system can not be obtained and each scheduler has only its local state, we propose a method to collect all the sequence of the local states of schedulers by sending them to a central observer component. 
%
The central observer then reconstructs a set of possible sequence of global states that could exists in the system.
%
The constructed sequence of global states is consumed by a runtime monitor.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Distributed CBSs with Multi-Party Interactions}
\label{sec:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Semantics of a Distributed CBSs with Multi-Party Interactions}
\label{subsec:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
A component-based system $B$ is a system whose behavior is obtained by composing the behavior of independent components $B_1, \ldots, B_n$.
%
\begin{definition}[Components of a CBS]
For $i \in [1,n]$, the behavior of component $B_i$ is defined as the labeled transition system (LTS) $( Q_i, \Actions_i \cup \setof{ \beta_i }, \trans{i}{} )$ such that:
%
\begin{itemize}
	\item $Q_i = Q_i^{\rm r} \cup Q_i^{\rm b}$ is the set of states,
	\item $\Actions_i$ is the set of actions,
	\item $\trans{i}{} \subseteq \left( Q_i^{\rm r} \times \Actions_i \times Q_i^{\rm b} \right) \cup \left( Q_i^{\rm b} \times \setof{\beta_i} \times Q_i^{\rm r} \right)$ is the set of transitions.
\end{itemize}   
%
Moreover, $Q_i$ has a partition $\setof{Q_i^{\rm r} , Q_i^{\rm b}}$ where $Q_i^{\rm r}$ (resp. $Q_i^{\rm b}$) is the so-called set of \emph{ready} (resp. \emph{busy}) states. 
%
\end{definition}
%
%
The set of ready (resp. busy) states $Q_i^{\rm r}$ (resp. $Q_i^{\rm b}$) is the set of states such that the component is ready (resp. not ready) to perform an action. %possibly joint with other components.
%
Component $B_i$ has (i) actions in set $\Actions_i$ which are possibly shared with some of the other components, and (ii) an action $\beta_i$ such that $\beta_i \notin \Actions$ which models internal computations of component $B_i$.
%
%As we shall describe below, the actions shared by several components are the so-called multi-party interactions, and schedulers ensure that they are jointly executed (\cf Definition~\ref{def:scheduler}).
%
\input{component_tank}
%
\begin{example}[Component]
\figref{fig:component} depicts a component Tank where, $\tank = ( Q^r \cup Q^b, \Actions \cup \setof{ \beta }, \trans{}{} )$ such that: 
%
\begin{itemize}
	\item[--] $Q^r= \setof{d,f}$ is the set of \emph{ready} states and $Q^b=\setof{d^\bot,f^\bot}$ is the set of \emph{busy} states,
	\item[--] $\Actions= \setof{\drain,\fil}$ is the set of actions and $\beta$ is the internal action,
	\item[--] $\trans{}{}= \setof{(d,\fil,d^\bot),(d^\bot,\beta,f),(f,\drain,f^\bot),(f^\bot,\beta,d)}$ is the set of transitions.
\end{itemize}
On the outer surface, each $\bullet$ represents an action and provides an interface for the component to synchronize with actions of other components in case of joint actions.
\end{example}
%
The system is endowed with a set of \emph{schedulers} $\setof{ S_1, \ldots, S_m}$ managing the execution of actions of components.
% are coordinated by a set of \emph{schedulers} $\mathcal{S} = \setof{ S_1, \ldots, S_m}$.
%
%It is known and given as one of the distributed system design criteria that which action is coordinated by which scheduler.
%
Identifying which action is coordinated by which scheduler is known and given as one of the distributed system design criteria.
%
As we shall describe below, the actions shared by several components are the so-called multi-party interactions (aka joint actions), and schedulers ensure that they are jointly executed (\cf Definition~\ref{def:scheduler}).
%
%Schedulers are used to coordinate the execution of components.
%
We assume a set of global actions used by the system $\Actions$ such that $\Actions \subseteq 2^{\cup^n_{i=1} \Actions_i}$ and $\forall a \in \Actions : |a \cap \Actions_i| \leq 1$.
%
Let us assume some auxiliary functions. 
%
\begin{itemize}
	\item[--] Function $\involved: \Actions \rightarrow 2^{[1,n]} \setminus \setof{\emptyset} $ indicates the components involved in actions.
%
Moreover, we extend function $\involved$ to internal actions by setting $ \involved(\beta_i) = i $, for any $ \beta_i \in \bigcup_{ i = 1 }^n$.
%
Action $a \in \Actions$ is a joint action if and only if $|\involved(a)| \geq 2$.
%
	\item[--] Function $\managed : \Actions \rightarrow S$ indicating the scheduler managing each action in the system such that for $a \in \Actions$, $\managed(a)=S_j$ if and only if action $a$ is coordinated by scheduler $S_j$.
%
	\item[--] Function $\scope : [1,m] \rightarrow 2^{[1,n]} \setminus \setof{ \emptyset }$ indicating the set of indexes of components in the scope of each scheduler such that $\scope(j) = {\displaystyle \bigcup_{a'\in \setof{a \in \Actions \mid \managed(a) = S_j}} \involved(a')}$.
	%
%	There exists at least one action for each component which is managed by the concerned scheduler.
\end{itemize}
%
%Schedulers are used to coordinate the execution of components.
%
%We assume a set of (independent) schedulers $\mathcal{S} = \setof{ S_1, \ldots, S_m}$, where a scheduler is modeled as follows:
%
\begin{definition}[Shared component]
The set of shared components is defined as
$B_s = \{ B_i \mid \exists j,k \in [1,m] :$ $ j \neq k \wedge i \in \scope(j) \cap \scope(k) \}$.
%
%
%Formally, the set of shared components is defined as
%$B_s = \setof{ B_i \mid j,k \in [1,m] : j \neq k \wedge i \in \scope(j) \cap \scope(k) }$.
\end{definition}
%
A shared component $B_i \in B_s$ is a component which is in the scope of more than one scheduler, that is, execution of the actions of $B_i$ are managed by more than one scheduler.
%
\begin{example}[Shared component]
\figref{fig:scheduler} depicts a component-based system consisting of three components each of which is an instance of the component in \figref{fig:component}. For $i \in [1,3]$, $\tank_i = ( Q_i^r \cup Q_i^b, \Actions_i \cup \setof{ \beta_i }, \trans{i}{} )$ with 
%
\begin{itemize}
	\item $Q_i^r= \setof{d_i,f_i}$, $Q_i^b=\setof{d^\bot_i,f^\bot_i}$,
	\item $\Actions_i= \setof{\drain_i,\fil_i}$,
	\item $\trans{i}{}= \setof{(d_i,\fil_i,d^\bot_i),(d^\bot_i,\beta_i,f_i),(f_i,\drain_i,f^\bot_i),(f^\bot_i,\beta_i,d_i)}$.
\end{itemize}
The set of global actions is $\Actions= \setof{ \setof{\drain_1}, \fil_{12}, \drain_{23}, \setof{\fil_3}}$ where $\fil_{12}= \setof{\fil_1,\fil_2}$ and $\drain_{23}= \setof{\drain_2,\drain_3}$ are joint actions.
%
Two schedulers $S_1$ and $S_2$ coordinate the execution of actions such that $\managed( \setof {\setof{\drain_1}, \fil_{12} })=S_1$ and $\managed( \setof{ \setof{\fil_3}, \drain_{23} })=S_2$.
%
Component $\tank_2$ is a shared component because action $\fil_{12}$ which is a joint action of $\fil_1$ and $\fil_2$ is coordinated by scheduler $S_1$ and the action $\drain_{23}$ which is a joint of $\drain_2$ and $\drain_3$ is coordinated by scheduler $S_2$. Consequently, component $\tank_2$ is in the scope of two schedulers and is a shared component. 
\end{example}
%
\begin{definition}[Scheduler]
\label{def:scheduler}
Scheduler $S_j \in \setof{S_1,\ldots,S_m}$
%The system is endowed with a set of schedulers $\setof{ S_1, \ldots, S_m}$ such that each scheduler $S_j$
is modeled by the LTS $( Q_{S_j}, \Actions_{S_j}, \trans{S_j}{})$ such that:
\begin{itemize}
	\item $Q_{S_i}$ is the set of states,
	%\item $2^{\Actions^\gamma_{S_j} \cup \Actions^\beta_{S_j}} \subseteq \Actions_{S_j} : \alpha \subseteq \Actions^\gamma_{S_j} , \beta \subseteq \Actions^\beta_{S_j}, (\alpha \cup \beta) \in \Actions_{S_j} , a_1,a_2 \in \alpha , \involved(a_1) \cap \involved(a_2) = \emptyset , \forall \beta_i \in \beta : \not \exists a \in \alpha , i \in \involved(a)$
	\item $\Actions_{S_j}$ is the set of actions of the scheduler $S_j$ such that $\Actions^\gamma_{S_j} \cup \Actions^\beta_{S_j}  \subseteq \Actions_{S_j}$ where $\Actions^\gamma_{S_j} \subseteq \Actions$ is the set of actions managed by $S_j$, that is $\Actions^\gamma_{S_j} = \setof{a \in \Actions \mid \managed(a) = S_j}$, $\Actions^\beta_{S_j}$ is the set of internal actions of the components involved in an action managed by $S_j$, that is $\Actions^\beta_{S_j} = \setof{\beta_i \mid i \in \scope(j)}$.
	%, and \\ $\Actions^{\gamma\beta_s}_{S_j} = \Actions^\gamma_{S_j} \cup \Actions^\beta_{S_j} \cup \beta_s$ with $\beta_s \subseteq  \Actions^\beta_{S_j}$ such that $\forall \beta_i \in \beta_s, \forall a \in \Actions^\gamma_{S_j} \cup \Actions^\beta_{S_j}, B_i \in B_s \wedge  \involved(\beta_i) \cap \involved(a)= \emptyset$ is the set of actions managed by $S_j$ and internal actions of shared components that can be trigger at the same time. 
	\item $\trans{S_j}{} \subseteq \left( Q_{S_j} \times \Actions_{S_j} \times Q_{S_j} \right)$ is the set of transitions.
\end{itemize}  
%
Moreover, $\forall a \in \Actions, \exists! j \in [1,m] : a \in \Actions_{S_j}$.
\end{definition}
%
%\begin{definition}[Scheduler]
%\label{def:scheduler}
%For all $i \in [1,m]$ the scheduler $S_i$ is modeled as an LTS $( Q_{S_i}, \Actions_{S_i}, \trans{S_i}{})$, where $Q_{S_i}$ is the set of states, $\Actions_{S_i}$ is the set of actions such that $\forall a \in \Actions, \exists! i \in [1,m] : a \in \Actions_{S_i}$ and $\trans{S_i}{} \subseteq \left( Q_{S_i} \times \Actions_{S_i} \times Q_{S_i} \right)$ is the set of transitions. 
%% $\forall a \in \Actions, \exists! s \in S: a \in \Actions_{s}$.
%\end{definition}
%
%
Intuitively, when a scheduler executes an action, it triggers the execution of this action on the involved components ready to execute this action.
%
Moreover, when a component executes internal action, it triggers the execution of the corresponding action on the associated schedulers and also sends the updated state of the component to the associated schedulers. 
%
%
%Furthermore, it is possible that at a moment a scheduler executes an action, it is also triggered by internal actions of shared components (associated to the scheduler).
%
Coordination of global actions of the system \ie $\Actions$, are distributed among schedulers. 
%
Actions of schedulers consisting of actions of the system, nevertheless each action of the system is associated to exactly one scheduler.
%
Consequently, schedulers manage disjoint sets of actions, such that $\forall i, j \in [1,m]: i \neq j \implies \Actions^\gamma_{S_i} \cap \Actions^\gamma_{S_j} = \emptyset$. 
%
%In the sequel, we shall assume some auxiliary function $\managed : \Actions \rightarrow S$ indicating the scheduler managing each action in the system and function $\scope : [1,m] \rightarrow 2^{[1,n]} \setminus \setof{ \emptyset }$ indicating the set of indexes of components in the scope of each scheduler such that there exists at least one action for each component which is managed by the concerned scheduler.
%
%
%For each component $B_{i \in [1,n]}$ in the scope of scheduler $S_{j \in [1,m]}$ there exists an action corresponding to the internal action of $B_i$, that is, each scheduler is aware of state updates of its associated components: $\forall j \in [1,m], \forall i \in \scope(j), \beta_i \in \Actions_{S_j}$, $\forall q \in Q_{S_j}, \exists q' , (q, \beta_i, q') \in \trans{S_j}{}$.
%
\input{scheduler}
%
\begin{example}[Scheduler]
In \figref{fig:scheduler},  for $j \in [1,2]$, scheduler $S_j = ( Q_{S_j}, \Actions_{S_j} , \trans{{S_j}}{} )$ with
\begin{itemize}
	\item $l_0, l_1, l_2 , l_3  \in Q_{S_j}$, 
	\item $ \Actions^\gamma_{S_1} = \setof{ \setof{\drain_1}, \fil_{12}}$, $\Actions^\beta_{S_1} = \setof{\beta_1, \beta_2}$ and $\Actions^\gamma_{S_2} = \setof{\drain_{23}, \setof{\fil_3}}$, $\Actions^\beta_{S_2} = \setof{\beta_2, \beta_3}$,
	%\item $(l_1, \fil_{12}, l_2), (l_2, \drain_1, l_1), (l_1, \beta_1, l_2), (l_1, \beta_2, l_2), (l_2, \beta_1, l_1), (l_2, \beta_2, l_1) \in \trans{{S_1}}{} $,
	\item $\{(l_0 , \beta_2 , l_0),(l_1 , \beta_2 , l_1),(l_1 , \beta_1 , l_0),(l_2 , \beta_2 , l_1),(l_3 , \beta_2 , l_0),(l_2 , \beta_1 , l_3),$ \\ $(l_3 , \drain_1 , l_2),(l_0 , \drain_1 , l_1),(l_0 , \fil_{12} , l_2)\}\in \trans{{S_1}}{}$,
%
%	
	%$\setof{(l , \beta_2 , l) \mid l \in Q_{S_1}}, (l_1, \setof{ \fil_{12}} , l_2 ), \setof{(l_2 , a , l_3),(l_4 , a , l_1) \mid a \in \setof{\{\beta_1\},\{\beta_1,\beta_2\}}} ,\hfill$ $\setof{(l_3, a , l_4) \mid a \in \setof{\setof{\drain_1}, \setof{\drain_1, \beta_2}}} \in \trans{{S_1}}{}$
	\item $\{(l_0 , \beta_2 , l_0),(l_1 , \beta_2 , l_1),(l_1 , \beta_3 , l_0),(l_2 , \beta_2 , l_1),(l_3 , \beta_2 , l_0),(l_2 , \beta_3 , l_3),$ \\ $(l_3 , \fil_3 , l_2),(l_0 , \fil_3 , l_1),(l_0 , \drain_{23} , l_2)\}\in \trans{{S_2}}{}$.
%
%	
	%$\setof{(l , \beta_2 , l) \mid l \in Q_{S_2}}, (l_3, \setof{ \drain_{23}} , l_4 ), \setof{(l_2 , a , l_3),(l_4 , a , l_1) \mid a \in \setof{\{\beta_3\},\{\beta_3,\beta_2\}}} ,\hfill$ $\setof{(l_1, a , l_2) \mid a \in \setof{\setof{\fil_3}, \setof{\fil_3, \beta_2}}} \in \trans{{S_2}}{}$
	%\item $(l_1, \fil_3, l_2), (l_2, \drain_{23}, l_1), (l_1, \beta_2, l_2), (l_1, \beta_3, l_2), (l_2, \beta_2, l_1), (l_2, \beta_3, l_1) \in \trans{{S_2}}{} $.
	
\end{itemize}
%
%\begin{itemize}
%	\item $\managed( \setof {\drain_1, \fil_{12} })=S_1$, 
%	\item $\managed( \setof {\fil_3, \drain_{23} })=S_2$.
%\end{itemize}
\end{example}
%
%
%
The global execution of the system can be described as the parallel execution of actions managed by the schedulers.
%
Moreover, the schedulers know when they have to execute an action.
%
\begin{definition}[Global behavior]
\label{def:global_behavior}
The global behavior of the system is the LTS $( Q , \GActions , \trans{}{}) $ where:
\begin{itemize}
	\item $Q \subseteq  \bigotimes_{i=1}^{n} Q_i \times \bigotimes_{j=1}^{m} Q_{S_j}$ is the set of states consisting of the states of schedulers and components,
	\item $\GActions = 2^{\Actions \ \cup\ \bigcup_{i \in [1,n]} \setof{\beta_i}}  \setminus \setof{ \emptyset } $ is the set of possible actions of the system consisting of either several shared actions and/or several internal actions (several actions can be executed concurrently by the system),
	\item  $\rightarrow \subseteq Q \times \GActions \times Q$ is the transition relation abiding to the following rule.   
	
%%
A transition is a move from state $( q_1, \ldots , q_n , q_{s_1} , \ldots , q_{s_m})$ to state $ ( q'_1, \ldots , q'_n ,  q'_{s_1} , \ldots , q'_{s_m}) $ on actions in set $ \alpha \cup \beta $, where $\alpha \subseteq \Actions$ and $\beta \subseteq \bigcup_{i \in [1,n]} \setof{ \beta_i } $, noted $ (  q_1, \ldots , q_n , q_{s_1} , \ldots , q_{s_m}) \longtrans{}{\alpha \cup \beta}$ $(  q'_1, \ldots , q'_n , q'_{s_1} , \ldots , q'_{s_m}) $, whenever the following conditions hold:
\begin{enumerate}
	\item
	$\forall j \in [1,m]: | \left( \alpha \cup \beta \right) \cap \Actions_{S_j} | \leq 1$,
	\item
	$\forall i \in [1,n]: | \left( \alpha \cap \Actions_i \right) \cup \left( \{ \beta_i \} \cap \beta \right) | \leq 1$,
	\item
	$ \forall a \in \alpha , \left( \left( \exists j \in [1,m]: \managed(a) = S_j \right) \Rightarrow \left( q_{s_j} \trans{S_j}{a} q'_{s_j} \wedge \forall i \in \involved(a) : q_i \longtrans{i}{a \cap \Actions_i} \ q'_i \right) \right) $,
		%
	\item
	$ \forall \beta_i \in \beta, q_i \longtrans{i}{\beta_i} \ q'_i $, $( i \in \scope(j) \Rightarrow q_{s_j} \longtrans{S_j}{\beta_i} q'_{s_j})$,
		%
	\item
	$ \forall i \in [1, n] \setminus \involved( \alpha \cup \beta ) : q_i = q'_i$,
	\item
	$ \forall j \in [1, m] \setminus \managed( \alpha ) : q_{s_j} = q'_{s_j}$. 
\end{enumerate}
%
	%
\begin{small}
			\begin{mathpar}
		\inferrule*
		{
%		   a \in \alpha \and  j\in[1,m]:\managed(a) = S_j \wedge q_{s_j} \longtrans{S_j}{a} q'_{s_j}  \and  k\in[1,m]: \not\exists a' \in \alpha, \managed(a') = S_k \wedge q_{s_k}=q'_{s_k} \\ \forall i \in \involved(a):q_i \longtrans{i}{a \cap \Actions_i}  q'_i \and \forall i \not\in \involved(a):q_i=q'_i \\  \forall i \in I : \beta_i \in \beta \and q_i \longtrans{i}{\beta_i}  q'_i \and \forall j \in [1,m] : i\in \scope(j) \wedge q_{s_j} \longtrans{S_j}{\beta_i} q'_{s_j} \and \forall i \not\in I \cup \involved(a):  q_i=q'_i
(1) \and (2) \and (3) \and (4) \and (5)
		}
		{
		    (  q_1, \ldots , q_n , q_{s_1} , \ldots , q_{s_m}) \longtrans{}{\alpha \cup \beta} (  q'_1, \ldots , q'_n , q'_{s_1} , \ldots , q'_{s_m})
		}
		\end{mathpar}
\end{small}
%
where functions $ \involved $ and $ \managed $ are extended to sets of (internal) actions in the usual way.
\end{itemize}
\end{definition}
%
The above rule allows the components of the system to execute independently according to the decisions of the
% independent
schedulers.
%
It can intuitively be understood as follows:
%
\begin{itemize}
	\item
Condition 1. states that a scheduler can trigger at most one action or can be triggered by at most one internal action at a time.
%
	\item
Condition 2. states that a component can perform at most one execution step at a time.
%
The set of executed actions ($ \alpha \cup \beta $) contains at most one action involving each component of the system.
%
	\item
Condition 3. states that whenever an action $a$ managed by scheduler $S_j$ is executed, $S_j$ and all components involved in this (multi-party inter)action must be ready to execute it.
%
	\item
Condition 4. states that internal actions are executed whenever the corresponding components are ready to execute them. Moreover, schedulers are aware of internal actions of components in their scope. Note that, awareness of internal actions of a component results transferring the updated state of the component to the schedulers. 
%
	\item
Conditions 5. and 6. state that the components and schedulers not involved in an action remain in the same state.
\end{itemize}
%
An example to illustrate the global behavior of the system depicted in~\figref{fig:scheduler} is provided later and described in terms of execution trace (\cf Example \ref{exmp:global_trace}).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Traces of a Distributed CBSs with Multi-Party Interactions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
At runtime, execution of a component-based system with multi-party interaction produces a global trace of events.
%
Intuitively, a global trace is the sequence of traversed states of the system, from some initial state and following the transition relation of the LTS of the system.
%
For the sake of simplicity and for our monitoring purposes, the states of schedulers are irrelevant in the trace and thus we restrict the global states to states of the components.
%
\begin{definition}[Global trace]
%
The global trace is the continuously-growing sequence $ ( q_1^0, \ldots , q_n^0 ) \cdot ( \alpha^0 \cup \beta^0 ) \cdot ( q_1^1, \ldots , q_n^1 )  \cdots ( q_1^k, \ldots , q_n^k ) \cdots $, such that $ q_1^0, \ldots , q_n^0 $ are the initial states of components of indexes $ 1, \ldots , n$ and $\forall i : (q_1^i, \ldots , q_n^i ) \longtrans{}{ \alpha^i \cup \beta^i } (q_1^{i+1}, \ldots , q_n^{i+1} ) $, where $\trans{}{}$ is the transition relation of the global behavior of the system and the states of schedulers are discarded.
%
%From some initial states $ q_1^0, \ldots , q_n^0 $ of components of indexes $ 1, \ldots , n$, the global trace is the continuously-growing sequence $ ( q_1^0, \ldots , q_n^0 ) \cdot ( \alpha^0 \cup \beta^0 ) \cdot ( q_1^1, \ldots , q_n^1 )  \cdots ( q_1^i, \ldots , q_n^n ) \cdots $ such that $\forall i : (q_1^i, \ldots , q_n^i ) \longtrans{}{ \alpha_i \cup \beta_i } (q_1^{i+1}, \ldots , q_n^{i+1} ) $, where $\trans{}{}$ is the transition relation defined above and the states of schedulers are discarded.
\end{definition}
%
Although the global trace of the system exists, it is generally not observable because it would require a perfect observer having simultaneously access to the states of the components.
%
Introducing such an observer (able to observe global states) in the system would require all components to synchronize, and would defeat the purpose of building a distributed system.
%
Instead of introducing such an observer, through instrumentation, it is possible to observe the sequence of states through schedulers.
%

Whenever the system produces a global trace $ t = ( q_1^0, \ldots , q_n^0 ) \cdot ( \alpha^0 \cup \beta^0 ) \cdot ( q_1^1, \ldots , q_n^1 )  \cdots $, each scheduler $ S_j $, $ j \in [ 1, m ] $, observes a local trace $ s_j (t) $ which consists in the sequence of state evolutions of the components it manages.
%
\begin{definition}[Local trace]
The local trace observed by scheduler $ S_j $ is inductively defined as follows:
\begin{itemize}
	\item 
	$ s_j \left( \left( q_1^0, \ldots , q_n^0 \right) \right) = \left( q_1^0, \ldots , q_n^0 \right) $, and
	\item
	$
	s_j \left( t \cdot ( \alpha \cup \beta ) \cdot \left( q_1, \ldots , q_n \right) \right)
	= \left\{
	\begin{array}{ll}
		t & \hbox{if } j \notin \managed( \alpha ) \wedge \involved ( \beta )\ \cap\ \scope ( j) = \emptyset \\
		t \cdot \gamma \cdot q' & \hbox{otherwise}
	\end{array}
	\right.
	$\\
	where
	\begin{itemize}
	\item
	$ \gamma =  \left( \alpha \ \cap\ \setof{ a \in \Actions  \mid \managed(a) = j } \right)\ \cup\ \left( \beta \cap \setof{ \beta_i \in \bigcup_{i=1}^n \setof{ \beta_i } \mid i \in \scope ( j ) } \right) $
	\item
	$ q' = ( q_1', \ldots , q_n' ) $ with 
	%$ q_i' = q_i $ if $ i \in \involved(\gamma) $ and $q_i' = ? $ otherwise.
	
	$
	q'_i
	= \left\{
	\begin{array}{ll}
		\last(s_j(t))_i & \hbox{if } i\not \in \involved ( \gamma ) \wedge i \in \scope ( j) \\
		q_i & \hbox{if } i \in \involved ( \gamma ) \wedge i \in \scope ( j) \\
		?  & \hbox{otherwise}(i \not\in \scope ( j ))
	\end{array}
	\right.
	$
	\end{itemize}
\end{itemize}
%
\end{definition}
%
We assume that the initial state of the system is observable by all the schedulers. 
%
An action $a \in \Actions$ is observable by scheduler $S_j$ if the action is managed by the scheduler $S_j$ that is $j \in \managed(a)$, also an internal action $\beta_{i \in [1,n]}$ is observable by scheduler $S_j$ if the associated component to the internal action $B_i$ is in the scope of the scheduler $S_j$, that is $i \in \scope(j)$. 
%
Observed state after an observable (internal) action consists of the states of components in the scope of $S_j$, that is $q_{i \in \scope(j)}$, and state of components out of the scope are said to be as unknown state (that is $?$). 
%
The auxiliary function $\last$ is defined such that 
for a local trace $s_j(t)=\left( q_1^0, \ldots , q_n^0 \right) \cdots \left( q_1^k, \ldots , q_n^k \right)$, $\last(s_j(t))_i=q_i^k$.
%
\begin{example}[Global trace and local trace]
\label{exmp:global_trace} 
Considering the system depicted in~\figref{fig:scheduler}, two possible global traces of such system is:\footnote{To simplify, we represent each busy state as $\bot$.}
\begin{itemize}
	\item $t_1=(d_1,d_2,d_3) \cdot \setof{\fil_{12}} \cdot (\bot, \bot, d_3) \cdot \setof{\beta_1} \cdot (f_1, \bot, d_3) \cdot \setof{\drain_1, \fil_3} \cdot (\bot, \bot , \bot ) \cdot \setof{\beta_2} \cdot (\bot, f_2 , \bot)$
	\item $t_2=(d_1,d_2,d_3) \cdot \setof{\fil_{12},\fil_3} \cdot (\bot, \bot, \bot) \cdot \setof{\beta_3} \cdot (\bot,\bot, f_3) \cdot \setof{\beta_2} \cdot (\bot, f_2 , f_3)\cdot \setof{\beta_1, \drain_{23}} \cdot (f_1, \bot , \bot )$
\end{itemize}
% 
Intuitively, $t_1$ and $t_2$ follow the global behavior of the system (Definition~\ref{def:global_behavior}).
%
In trace $t_1$, execution of action $\fil_{12}$ represents simultaneous execution of action $\fil_{12}$ in scheduler $S_1$, action $\fil_1$ in component $\tank_1$ and action $\fil_2$ in component $\tank_2$.
%
After $\fil_{12}$, component $\tank_1$ and $\tank_2$ go to their busy state whereas state of component $\tank_3$ remains unchanged.
%
Moreover, $\beta_2$ in trace $t_1$ represents simultaneous execution of action $\beta_2$ in component $\tank_2$, action $\beta_2$ in scheduler $S_1$ and action $\beta_2$ in scheduler $S_2$.
%
After $\beta_2$, component $\tank_2$ goes to its ready state \ie $f_2$.
%
In trace $t_2$, execution of two actions $\fil_{12}$ and $\fil_3$ represents simultaneous execution of action $\fil_{12}$ in scheduler $S_1$, action $\fil_3$ in scheduler $S_2$, action $\fil_1$ in component $\tank_1$ and action $\fil_2$ in component $\tank_2$ and action $\fil_3$ in component $\tank_3$. Trace $t_2$ ends up with simultaneous execution of action $\drain_{23}$ and internal action of component $\tank_1$.

the associated local observed traces are: 
%
\begin{itemize}
	\item $s_1(t_1)= (d_1,d_2,d_3) \cdot \setof{\fil_{12}} \cdot (\bot, \bot, ?) \cdot \setof{\beta_1} \cdot (f_1, \bot, ?) \cdot \setof{\drain_1} \cdot (\bot, \bot, ?) \cdot \setof{\beta_2} \cdot (\bot, f_2 , ?)$
	\item $s_2(t_1)= (d_1,d_2,d_3) \cdot \setof{\fil_3} \cdot (?, d_2, \bot) \cdot \setof{\beta_2} \cdot (?, f_2 , \bot)$
	%
	\item $s_1(t_2)= (d_1,d_2,d_3) \cdot \setof{\fil_{12}} \cdot (\bot, \bot, ?) \cdot \setof{\beta_2} \cdot (\bot, f_2, ?) \cdot \setof{\beta_1} \cdot (f_1, f_2, ?)$
	\item $s_2(t_2)= (d_1,d_2,d_3) \cdot \setof{\fil_3} \cdot (?, d_2, \bot) \cdot \setof{\beta_3} \cdot (?, d_2, f_3) \cdot \setof{\beta_2} \cdot (?, f_2, f_3)\cdot \setof{\drain_{23}} \cdot (?, \bot, \bot)$
\end{itemize}
\label{xmp:dmodel}
\end{example}
%
%Note that, at one time instance a scheduler could only execute one action but it could be be aware of several internal actions. 
%

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{From Local Traces to Global Traces}
\label{sec:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\paragraph{Central observer:}
\input{observer}
%
We define a new component as a \textit{passive} observer which runs in parallel with the system and collects  local traces of schedulers as its shown in~\figref{fig:observer}. Observer is always ready to receive information from schedulers. 
%
We use term \textit{passive} for our proposed observer since it does not force schedulers to send data. 
%
%
\begin{definition}[Observer]
The behavior of observer $\mathcal{O}$ can be modeled as an LTS $( Q_{\mathcal{O}}, \Actions_{\mathcal{O}}, \trans{\mathcal{O}}{})$ such that
\begin{itemize}
	\item $Q_{\mathcal{O}}$ is the set of states,
	\item $\Actions_{\mathcal{O}}$ is the set of actions where, $\forall a \in {\Actions \ \cup\ \bigcup_{i \in [1,n]} \setof{\beta_i}},\exists a' \in \Actions_{\mathcal{O}}$,
	\item $\trans{\mathcal{O}}{} \subseteq Q_{\mathcal{O}} \times \Actions_{\mathcal{O}} \times Q_{\mathcal{O}}$ is the set of transitions.
\end{itemize}
\end{definition}
%
%\begin{definition}[Observer]
%$( Q_{\mathcal{O}}, \Actions_{\mathcal{O}}, \trans{\mathcal{O}}{})$.
%\begin{itemize}
%	\item $\forall a \in \Actions, (a,\VC) \in \Actions_{\mathcal{O}}, \forall  q \in Q_{\mathcal{O}},\exists q', (q, (a,\VC) ,q') \in \longtrans{\mathcal{O}}{} $ where $\VC \in V$.
%	\item $\forall i \in [1,n],  \exists q \longtrans{\mathcal{O}}{(\beta_i,q_i)} q' : q,q' \in Q_{\mathcal{O}}, q_i \in Q^r_i$
%\end{itemize}
%\end{definition}
%
%
For each (internal) action of a system there exists a corresponding  action in the observer.  
%
We shall prove that such observer does not affect the semantics and performance of the distributed system (\cf Proposition~\ref{proposition:sim}).
%

For monitoring purposes, it is required that the observer be able to order actions execution of different received local traces appropriately. 
%
%A fundamental necessity in our distributed model for monitoring purposes is that observer be able to order their incoming messages appropriately. 
%
This need presents itself in the basic operating logic of a distributed computation such as retrieving a global view on the computation that represents a consistent global system state.
%
%This need presents itself in the basic operating logic of a distributed computation as well as in higher level applications such as retrieving a global view on the computation that represents a consistent global system state.
%
Since schedulers in our abstract model, do not interact directly together through sending/receiving messages, execution of an action in one scheduler seems to be concurrent with execution of all actions of other schedulers.   
%
Nevertheless, if schedulers $S_j$ manages action $a$ and $S_k$ manages action $b$ such that a shared component $B_i \in B_s$  is involved in $a$ and $b$, \ie  $i \in \involved(a) \cap \involved(b)$, as a matter of fact, execution of actions $a$ and $b$ are causally related.
%
In other words, there exists only one possible ordering of $a$ and $b$ and they could not have been executed concurrently.
%
Ignoring the actual ordering of $a$ and $b$ results  retrieving inconsistent global view. 
%

Lamport introduced logical clocks as a device to substitute for a global real time clock.
%
Logical clocks are used to order events (actions execution) based on their relative logical dependencies rather than on a ``time'' in the common sense. 
%
Vector clocks are a more powerful extension of Lamport's scalar logical clocks.
% 
\begin{definition}[Vector clock]
Vector clock $\VC$ is a vector of $m$ scalar (initially zero) values $c_1,\ldots,c_m$ locally stored in each scheduler $S_j$ where for all $k \in [1,m]$, $\VC(k)=c_k$ holds the latest (scalar) clock value scheduler $S_j$ knows from scheduler $S_k$.
\end{definition}
%
\begin{example}[Vector clock]
Let consider the global trace $t_2$ in Example \ref{exmp:global_trace}.
%
$\VC_1$ and $\VC_2$ denote vector clocks of scheduler $S_1$ and $S_2$ respectively.
%
Initially $\VC_1=\VC_2=(0,0)$.
%
After the simultaneous execution of $\fil_{12}$ and $\fil_3$, vector clocks are updated to $\VC_1=(1,0)$ and $\VC_2=(0,1)$.
%
Comparing $\VC_1$ and $\VC_2$ results the parallelism between  $\fil_{12}$ and $\fil_3$, which means that each of $\fil_{12}$ and $\fil_3$ could happened either before or after the other.
%
Since each of the schedulers has no information about the execution of the other one, they just are able to update the clock associated to their own.
%
Execution of $\drain_{23}$ results $\VC_2=(1,2)$ which means that scheduler $S_2$ knows that $\fil_{12}$ already executed by scheduler $S_1$, because a shared component, \ie $\tank_2$, is involved in both $\fil_{12}$ and $\drain_{23}$.
\end{example}
%
In the following, we instrument our abstract distributed system to let schedulers to send their local traces to the observer.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Composing with controller}
\label{sec:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Given a distributed system consisting of a set of component $B_1,\ldots, B_n$ and schedulers $S_1,\ldots, S_m$ where $S_j=( Q_{S_j}, \Actions_{S_j}, \trans{s_j}{})$, for all $j \in [1,m]$, we attach a local controller $\mathcal{C}^s_j$ in charge of computing the vector clock and sending local trace of $S_j$ to the observer.
%
Controller $\mathcal{C}^s_j$ is designed to compute the correct vector clock of scheduler $S_j$ through the shared components.
%
%
\begin{definition}[Scheduler controller]
Controller $\mathcal{C}^s_j$ is defined by a 3-tuple $( L \times 2^{[1,n]} \times V, \mathcal{R} , \trans{c^s_j}{})$ and is represented as a deterministic automaton depicted in \figref{fig:controller_scheduler}.
%
\begin{itemize}
	\item $L = \setof{ l_{req}, l_{resp}}$ is set of locations,
	%\item $2^{[1,n]}$ is the set of busy components which their latest action is coordinated by scheduler $S_i$,
	\item $V$ is set of vector clocks,
	\item $\mathcal{R}=\setof {\inc} \cup \setof { \req_i , \res_i , upd_i \mid i \in [1,n] ,\scope(j) \cap i \neq \emptyset, B_i \in B_s }$ is the set of actions.
%
%	Action $inc$ corresponds to increment local clock upon execution of an action managed by $S_i$, $req_j$ corresponds to request for updated vector clock upon receipt a request, $res_j$ corresponds to respond to a request and $upd_j$ corresponds to update the vector clock.
%
	\item $\trans{c^s_j}{}$ is the transitions defined as $\trans{c^s_j}{}= \tau_1 \cup \tau_2 \cup \tau_3 \cup \tau_4$, with 
\begin{itemize}
	\item  $\tau_1 = \Bigg\{(l, \mathcal{I},\VC)\longtrans{c^s_j}{inc}(l, \mathcal{I}',\VC') \mid \exists (q,a,q')\in \trans{s_j}{}, a\in \Actions, \mathcal{I}'=\mathcal{I} \cup \involved(a),$ $\VC'(j)=\VC(j)+1, l \in L \Bigg\}$.
	%
	\item  $\tau_2 = \Bigg\{(l, \mathcal{I},\VC) \longtrans{c^s_j}{\beta_i}(l, \mathcal{I'},\VC) \mid \exists (q,\beta_i,q')\in \trans{s_j}{} , B_i \not \in B_s , \mathcal{I}'= \mathcal{I} \setminus \setof{i}, l \in L \Bigg\}$.
	%
%	For all transitions associated to execution of an action in scheduler $S_i$, there exists an action in controller $\mathcal{C}^s_i$ to update local clock.
	%
	\item  $\tau_3 = \Bigg\{(l_{\req}, \mathcal{I},\VC) \longtrans{c^s_j}{\req_i}(l_{\res}, \mathcal{I}',\VC) , (l_{\res}, \mathcal{I}',\VC) \longtrans{c^s_j}{(\res_i, \VC)}(l_{\req}, \mathcal{I}',\VC),$ \\ $(l_{\req}, \mathcal{I}',\VC)  \longtrans{c^s_j}{\beta_i}  (l_{\req}, \mathcal{I}',\VC) \mid \exists (q,\beta_i,q')\in \trans{s_j}{} , B_i \in B_s , i \in \mathcal{I}, \mathcal{I}'= \mathcal{I} \setminus \setof{i} \Bigg\}$.
	%
%	For each transition associated to awareness of internal action of a shared component in which $S_i$ coordinated its latest action, there exists an input/output action  in controller $\mathcal{C}^s_i$ to exchange vector clock between scheduler and the shared component.
	%
	\item  $\tau_4 = \Bigg\{(l, \mathcal{I},\VC) \longtrans{c^s_j}{(upd_i, \VC')}(l, \mathcal{I},\VC'') \mid \exists (q,\beta_i,q')\in \trans{s_j}{} , B_i \in B_s , i \not \in \mathcal{I},$\\ $\VC''(k)=\max (\VC(k), \VC'(k)), k\in [1,m], l \in L \Bigg\}$.
	%
%	For each transition associated to awareness of internal action of a shared component in which $S_i$ did not coordinate its latest action, there exists an action  in controller $\mathcal{C}^s_i$ to update the vector clock of $S_i$. 
	%
\end{itemize}
\end{itemize}
\end{definition}
%
\begin{itemize}
	\item Action $\inc$ corresponds to increment local clock upon execution of an action managed by $S_j$, $\req_i$ corresponds to request for updated vector clock upon receipt a request, $\res_i$ corresponds to respond to a request and $upd_i$ corresponds to update the vector clock.
	\item For all transitions associated to execution of an action in scheduler $S_j$, there exists an action in controller $\mathcal{C}^s_j$ to update local clock ($\tau_1$).
	%
	\item For each transition associated to the awareness of the internal actions of non-shared components in scheduler $S_j$, there exists an action in controller $\mathcal{C}^s_j$ to send the updated state to the observer ($\tau_2$).
	%	
	\item For each transition associated to awareness of internal action of a shared component in which $S_j$ coordinated its latest action, there exists a request/response action in controller $\mathcal{C}^s_j$ to exchange vector clock between scheduler and the shared component.
	%
	Moreover, each request/response actions is followed by another action which is dedicated to send the updated state to the observer ($\tau_3$).
	%
	\item For each transition associated to awareness of internal action of a shared component in which $S_j$ did not coordinate its latest action, there exists an action  in controller $\mathcal{C}^s_j$ to update the vector clock of $S_j$ ($\tau_4$).
	%
\end{itemize}		
%
\input{scheduler_controller}
%
%For all transitions associated to execution of an action in scheduler $S_i$, there exists a action in controller $\mathcal{C}_i$ to update local clock (\ie $\tau_1$). 
%%
%For each transition associated to awareness of internal action of a shared component in which $S_i$ coordinated its latest action, there exists an input/output action  in controller $\mathcal{C}_i$ to exchange vector clock between scheduler and the shared component (\ie $\tau_2$).
%%
%For each transition associated to awareness of internal action of a shared component in which $S_i$ did not coordinate its latest action, there exists an action  in controller $\mathcal{C}_i$ to update the vector clock of $S_i$ (\ie $\tau_3$). 
%
Note that, latter we augment each shared component to store a vector clock and be able to send request and receive response. 
%

The composition of scheduler and controller is noted $S_j \otimes \mathcal{C}^s_j$.
%
%For each action of scheduler $S_i$ associated to the internal action of a shared component which $S_i$ coordinated its latest action, controller $\mathcal{C}_i$ has two transitions, a request transition which is a request notification from that shared component and an update transition which is a response of the request.  
\begin{definition}[Semantics of $S_j \otimes \mathcal{C}^s_j$]
The composition $S_j \otimes \mathcal{C}^s_j$ is the LTS $(Q_{S_j} \times L \times 2^{[1,n]} \times V, \Actions_{S_j} \cup \mathcal{R}, \trans{sc_j}{} )$ where the transition relation $\trans{sc_j}{}$ is defined by the following semantics rules:
%
\begin{enumerate}
	\item 
	%Execution of an action $a\in \Actions$ updates the vector clock by increasing the local clock and set of busy components. Updated state is sent to the observer.
		\begin{mathpar}
		\inferrule*
		{
		   a\in \Actions \and  q \longtrans{s_j}{a} q'  \and (l , \mathcal{I},\VC)\longtrans{c^s_j}{inc}(l , \mathcal{I}',\VC')
		}
		{
		   (q,l,\mathcal{I},\VC) \longtrans{sc_j}{a/(a , \VC')} (q',l,\mathcal{I}',\VC')
		}
		\end{mathpar}
		
%	\item 
%		\begin{mathpar}
%		\inferrule*
%		{
%		   a\in \Actions \and  q \longtrans{s_i}{a} q'  
%		}
%		{
%		   (q,\mathcal{I},\VC) \longtrans{sc_i}{\epsilon/a} (q',\mathcal{I}',\VC')
%		}
%		\end{mathpar}

	\item 
	%Awareness of an internal action  of component $B_j$ where $j \in \mathcal{I}$, requires transferring vector clock of $S_i$ to $B_j$. Updated state is sent to the observer after all. 
		\begin{mathpar}
		\inferrule*
		{
		   (l_{\req}, \mathcal{I},\VC) \longtrans{c^s_j}{\req_i}(l_{\res}, \mathcal{I}',\VC)
		}
		{
		   (q,l_{\req},\mathcal{I},\VC) \longtrans{sc_j}{\req_i / \epsilon} (q,l_{\res},\mathcal{I}',\VC)
		}
		\end{mathpar}
	\item  
		\begin{mathpar}
		\inferrule*
		{
		 (l_{\res},\mathcal{I},\VC) \longtrans{c^s_j}{(\res_i, \VC)}(l_{\req},\mathcal{I}',\VC)
		}
		{
		   (q,l_{\res},\mathcal{I},\VC) \longtrans{sc_j}{\epsilon/(\res_i, \VC) } (q,l_{\req},\mathcal{I}',\VC)
		}
		\end{mathpar}
	\item  
		\begin{mathpar}
		\inferrule*
		{
		   j \in \mathcal{I} \and  q \longtrans{s_j}{\beta_i} q'  \and (l, \mathcal{I},\VC) \longtrans{c^s_j}{\beta_i}(l, \mathcal{I'},\VC) 
		}
		{
		   (q,l,\mathcal{I},\VC) \longtrans{sc_j}{\beta_i / \beta_i} (q',l,\mathcal{I'},\VC)
		}
		\end{mathpar}
			\item 
			%Scheduler $S_j$ does not send information to the observer after receiving state update of a shared component $B_j$ in which its latest action was not coordinated by the scheduler $S_i$. Awareness of an internal action  of component $B_j$ just update the vector clock of $S_i$.  
		\begin{mathpar}
		\inferrule*
		{
		   i \not\in \mathcal{I} \and  q \longtrans{s_j}{\beta_i} q'   \and (l,\mathcal{I},\VC) \longtrans{c_j}{(upd_i,\VC') / \epsilon}(l,\mathcal{I},\VC'')
		}
		{
		   (q,l,\mathcal{I},\VC) \longtrans{sc_j}{(\beta_i,\VC') / \epsilon} (q',l,\mathcal{I},\VC'')
		}
		\end{mathpar}
%			\item 
%		\begin{mathpar}
%		\inferrule*
%		{
%		   j \in \mathcal{I} \and  q \longtrans{s_i}{\beta_j} q'
%		}
%		{
%		   (\mathcal{I},\VC) \longtrans{c_i}{pre / upd} (\mathcal{I},\VC)
%		}
%		\end{mathpar}
%
%
%	\item  $V$ is a set of vector clocks and $2^{[1,n]}$ is a set of indexes of components.
	%\item A single action $\setof{o}$ is added to the set of all actions of the scheduler which is associated to sending updated state information to the observer.
	%\item Transition relations are augmented by a new set of transitions $\obs{S_i}{}$. 
%	\item Transition associated to the execution of an action, \ie $a \in \Actions$, $q \trans{s_i}{a} q'$ where $q,q' \in Q_{S_i}$, are replaced by an input/output transition:	
%$\left( q,\mathcal{I},(c_1,\ldots,c_i,\ldots,c_m) \right) \longtrans{s_i}{a/a} \left( q',\mathcal{I} \cup \involved(a),(c_1,\ldots,c_i+1,\ldots,c_m)\right)$, where $\mathcal{I}$ is the set of indexes of currently executing components executed by scheduler $S_i$. 
%	\item Transitions associated to the awareness of internal action of components $B_j: j \in \mathcal{I}$ are replaced by an input/output action:
%		\begin{mathpar}
%		\inferrule*
%		{
%		   j \in \mathcal{I} \and  q \longtrans{s_i}{\beta_j} q'  
%		}
%		{
%		   (q,\mathcal{I},(c_1,\ldots,c_m)) \longtrans{s_i}{\beta_j / \beta_j} (q',\mathcal{I} \setminus \setof{j},(c_1,\ldots,c_m))
%		}
%		\end{mathpar}
% 
\end{enumerate}
%
Transition $\longtrans{sc_j}{a/b}$ in composition $S_j \otimes \mathcal{C}^s_j$ is denoted as an Input/Output transition in which $a$ (\resp $b$) is associated to an action to receive data (\resp to send data). 
%
% transition is an extension of transition $\longtrans{s_j}{a}$ in $S_j$ such that action $b$ is associated to sending information, whether to the observer or to a shared component.   
%
\end{definition}
%
The above rules can be intuitively be understood as follows:
\begin{itemize}
	\item Rule (1). Execution of an action $a\in \Actions$ updates the vector clock by increasing the local clock and also updates the set of busy components (that is $\mathcal{I}$). Observer get notified of execution of $a$ and the associated vector clock.
	%
	\item Rules (2,3). Receiving a request is followed by the response transferring the updated vector clock to the component which has sent the request.
	%
	\item Rule (4). Awareness of an internal action of component $B_i$ where $i \in \mathcal{I}$ (that is, the informed scheduler has managed the latest action of component $B_i$), transfers the updated state of component $B_i$ to the observer. 
	%
	\item Rule (5). Scheduler $S_j$ does not send information to the observer after receiving state update of a shared component $B_i$ in which its latest action was not coordinated by the scheduler $S_j$. Awareness of an internal action  of component $B_i$ just update the vector clock of $S_j$.  
\end{itemize}
%
\input{shared_comp_controller}
%
Moreover, to each shared component $B_i \in B_s$, we attach a local controller in order to exchange the vector clock among schedulers in the set $\setof{S_j \mid j\in [1,m], \scope(j) \cap i \neq \emptyset}$. 
%
\begin{definition}[Shared component controller]
Local controller $\mathcal{C}^b_i$ for a shared component $B_i \in B_s$ with the behavior $( Q_i, \Actions_i \cup \setof{ \beta_i }, \trans{i}{} )$ is formally defined by a 3-tuple $(L \times [1,m] \times V,\mathcal{R}, \trans{c^b_i}{})$ and presented as a deterministic automaton depicted in \figref{fig:controller_shared_component}, where


%For each shared component $B_i \in B_s$ with the behavior $( Q_i, \Actions_i \cup \setof{ \beta_i }, \trans{i}{} )$, we attach a local controller $\mathcal{C}_i$ which is defined as a deterministic automaton depicted in \figref{fig:controller_shared_component} and represented formally by a 3-tuple $(L \times [1,m] \times V,\mathcal{R}, \trans{c_i}{})$ in order to exchange the vector clock among schedulers in the set $\setof{S_j \mid j\in [1,m], \scope(j) \cap i \neq \emptyset}$. 
%
\begin{itemize}
	\item $L = \setof{ l_{new}, l_{req}, l_{resp}}$ is set of locations,
	\item $V$ is the set of vector clocks,
	\item $\mathcal{R}=\setof{new} \cup \setof{\req_j,\res_j \mid j\in [1,m],\scope(j) \cap i \neq \emptyset}$ is the set of actions, 
	\item $\trans{c^b_i}{}$ is the transitions defined as $\trans{c^b_i}{}= \tau_1 \cup \tau_2$, with 

%$\trans{c_i}{}$ is the transitions defined as $\trans{c_i}{}= \tau_1 \cup \tau_2$, with 
	%\item $\tau_1 = \setof{(j, \VC) \longtrans{c_i}{*}(j', \VC) \mid \exists (q,a,q')\in \trans{i}{} , a\in \Actions,  j'= \managed(a)}$
\begin{itemize}
	\item $\tau_1 = \setof{(l_{new},j, \VC) \longtrans{c^b_i}{new}(l_{req},\managed(a), \VC) \mid a \in \Actions, (q,a,q')\in \trans{i}{} }$
	\item $\tau_2 = \Bigg\{ (l_{\req},j, \VC) \longtrans{c^b_i}{\req_j}(l_{\res},j, \VC), (l_{\res},j, \VC) \longtrans{c^b_i}{(\res_j,\VC')}(l_{new},j, \VC'') \mid$\\ $\exists (q,\beta_i,q')\in \trans{i}{}, \VC''(k)=\max (\VC(k), \VC'(k)), k\in [1,m]\Bigg\}$ 
\end{itemize}
\end{itemize}
\end{definition}
%
\begin{itemize}
	\item For each transition in the component $B_i$ associated to execution of an action $a$, the exists a transition in  $\mathcal{C}^b_i$ which keeps the index of the scheduler which executed $a$ ($\tau_1$). 
	%
	\item For each transition in the component $B_i$ associated to execution of the internal action $\beta_i$, there exists a request/response action in  $\mathcal{C}^b_i$ to obtain the updated vector clock of the scheduler which managed the latest actions of $B_i$ ($\tau_2$).
\end{itemize}
%
The composition of shared component $B_i \in B_s$ and controller is noted $B_i \otimes \mathcal{C}^b_i$. 
%
\begin{definition}[Semantics of $B_i \otimes \mathcal{C}^b_i$]
The composition $B_i \otimes \mathcal{C}^b_i$ is the LTS $(Q_i \times L \times [1,m] \times V, \Actions_i \cup \setof{\beta_i} \cup \mathcal{R}, \trans{bc_i}{} )$ where the transition relation $\trans{bc_i}{}$ is defined by the following semantics rules:
\begin{enumerate}
	\item 
	%Execution of an action $a\in \Actions$, updates the variable associated to the index of the scheduler which did $a$. 
			\begin{mathpar}
		\inferrule*
		{
		   a \in \Actions \and q \longtrans{i}{a} q' \and (l_{new},j, \VC) \longtrans{c^b_i}{new}(l_{\req},\managed(a), \VC)
		}
		{
		   (q,l_{new}, j, \VC) \longtrans{bc_i}{a} (q',l_{\req}, \managed(a), \VC)
		}
		\end{mathpar}
		%
		\item 
%	Execution of internal action sends a request to obtain the updated the vector clock.
			\begin{mathpar}
		\inferrule*
		{
		   q \longtrans{i}{\beta_i} q'  
		}
		{
		   (q,l_{\req}, j, \VC) \longtrans{bc_i}{\req_j /(\res_j ,\VC') / \beta_i} (q',l_{new}, j, \VC'')
		}
		\end{mathpar}
%	\item 
%%
%			\begin{mathpar}
%		\inferrule*
%		{
%		   q \longtrans{i}{\beta_i} q' \and (l_{req}, j, \VC) \longtrans{c^b_i}{req_j}(l_{resp}, j, \VC) 
%		}
%		{
%		   (q,l_{req}, j, \VC) \longtrans{bc_i}{\beta_i / req_j} (q',l_{resp}, j, \VC)
%		}
%		\end{mathpar}
%	\item 
%	%
%			\begin{mathpar}
%		\inferrule*
%		{
%		   (l_{resp}, j, \VC) \longtrans{c^b_i}{(resp_j,\VC')}(l_{new}, j, \VC'')
%		}
%		{
%		   (q,l_{resp}, j, \VC) \longtrans{bc_i}{(resp_j,\VC') /\beta_i} (q,l_{new}, j, \VC'')
%		}
%		\end{mathpar}
%	%\item for all $q \longtrans{i}{a} q' : \managed(a)=j$ last executed scheduler id is set to $j$. 
%	%\item for all $q \longtrans{i}{\beta_i} q'$, there exists set of transitions in controller: 
%%	\begin{itemize}
%%		\item $\VC \longtrans{c_i}{req_j} \VC$
%%		\item $\VC \longtrans{c_i}{upd_j} \VC'$
%%		\item $\setof{\VC \longtrans{c_i}{\beta_{ik}} \VC \mid k \in [1,m] \wedge \scope(k) \cap i \neq \emptyset \wedge k \neq j}$
%%					\begin{mathpar}
%%		\inferrule*
%%		{
%%		   q \longtrans{i}{\beta_i} q' 
%%		}
%%		{
%%		   (q, \VC, k) \longtrans{c_i}{\beta_i} (q', \VC, k)
%%		}
%%		\end{mathpar}
%%	\end{itemize} 
\end{enumerate}
%
%Input/Output/Output transition $\longtrans{bc_i}{a/b}$ in composition $B_i \otimes \mathcal{C}^b_i$ is an extension of transition $\longtrans{i}{a}$ in $B_i$ such that action $b$ is associated to sending information to associated schedulers.  
%
Transition $\longtrans{sc_j}{a/b/c}$ in composition $B_i \otimes \mathcal{C}^b_i$ is denoted as an Output/Input/Output transition in which $a$ (\resp  $c$) is associated to request action (\resp notification action which sends data) and $b$ is associated to an action to receive data. 
\end{definition}
%
The above rules can be intuitively be understood as follows:
\begin{itemize}
	\item Rule (1). Execution of an action $a\in \Actions$, updates the variable associated to the index of the scheduler which did $a$.
	\item Rule (2). Execution of internal action sends a request to obtain the updated the vector clock. Receiving the response of the request, updates the vector clock and sends the updated state to the associated schedulers.
%	\item Rule (3). Receiving the response of the request, updates the vector clock and sends the its state to the associated schedulers.
\end{itemize}
%
\begin{proposition}
\label{proposition:sim}
$(S_1,\ldots,S_m,B_1,\ldots,B_n) \sim (S_1 \otimes \mathcal{C}^s_1,\ldots,S_m \otimes \mathcal{C}^s_m,B'_1,\ldots,B'_n,\mathcal{O})$ where $\forall j \in [1,n], B'_j = B_j \otimes \mathcal{C}^b_j$ if $B_j \in B_s$ and $B'_j = B_j$ otherwise.
\end{proposition}
%
Proposition~\ref{proposition:sim} states that observed system is bisimilar to the initial system and the semantic of initial system is preserved in the observed system. 
%
\begin{definition}[Sequence of events]
We define $\mathcal{U}$ as a set of sequences of received updates (aka event).
%
Formally, $\mathcal{U}= \setof{u_1 \cdot u_2 \cdot u_3 \cdots \mid i >0 , u_i \in \setof{(a,\VC) \mid a \in \Actions , \VC \in V} \cup \setof{(\beta_j, q_j) \mid j\in [1,n], q_j \in Q_j}}$.
\end{definition}
%
\begin{example}
Considering Example~\ref{xmp:dmodel}, following are the sequence of information to be sent to the observer from each scheduler.
\begin{itemize}
	\item trace $t_1$,
	\begin{itemize}
		\item $S_1 : (\fil_{12},(1,0)) \cdot (\beta_1,f_1).(\drain_{23},(2,0)) \cdot (\beta_2,f_2)$
		\item $S_2 : (\fil_3,(0,1))$
	\end{itemize}
	\item trace $t_2$,
	\begin{itemize}
		\item $S_1 : (\fil_{12},(1,0)) \cdot (\beta_2,f_2) \cdot (\beta_1,f_1)$
		\item $S_2 : (\fil_3,(0,1)) \cdot (\beta_3,f_3) \cdot (\drain_{23},(1,2))$
	\end{itemize}
\end{itemize}
$S_2$ is aware of state update $(\beta_2,f_2)$ but it does not sent it to the observer, based on the semantics rules,  scheduler $S_i$ only sends the received states of a component if the latest execution of the component has been coordinated by $S_i$.
\end{example}
%
To interpret the states updates received by the observer we use the notion of computation lattice.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Computation Lattice of a Distributed CBSs with Multi-party Interactions}
\label{sec:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Computation lattice of a distributed system is represented in a form of $m$ orthogonal axes.
%
Each axis dedicated for evolution of system in a specific scheduler.
%
Computation lattice expresses all the possible traces in the distributed system.
%
Each path in the lattice represent a global trace of the system that could possibly have happened.
%

%\paragraph{From observed local traces to lattice:}
%The naive way to build the computation lattice by receiving state updates from schedulers is to start extending lattice (initially from the initial state) in the direction of axis associated to the scheduler which sent its state.
%
We represent the lattice implicitly using vector clocks.
%
We propose an on-the-fly method to generate the computation lattice at runtime which consists of two steps, \textit{extending-joint making} and \textit{updating} of lattice. 
%
Sending information from schedulers to the observer is an \textit{event}.
%
Events regarding to the execution of an action in any scheduler (\ie $E_a = \setof{(a,\VC) \mid a \in \Actions, \VC \in V}$), extends the lattice in the associated direction (\ie direction of evolution of $S_i$ where $i=\managed(a)$). 
%
Events regarding to the internal actions (\ie $E_\beta= \setof{(\beta_j,q_j) \mid j \in [1,n], q_j \in Q_j}$, updates those nodes of the lattice which have busy state of component corresponding to the internal action.
%
%Formally, computation lattice $\mathcal{L}$ of a distributed system is defined as a tuple of set nodes  and happened-before relation, $\mathcal{L}=(Q \times V,\rightarrowtail)$.
%
Since reception of events are not totally ordered due to communication delay, we extend the lattice based on vector clocks attached to each event.
%
%A vector $\VC=(c_1,\dots,c_m)$ is the vector clock locally stored in scheduler $S_{j \in [1,m]}$. 
%
%For all $k\in[1,m]$, $\VC(k)=c_k$ is the value of logical clock of scheduler $S_k$, as per the knowledge of scheduler $S_j$. 
%
%In other words, $S_j.\VC(k)=z$, implies that scheduler $S_j$ is aware of occurrence of $z^{\rm th}$ action in $S_k$.
%
%Execution of each action is labeled by a specific and unique vector clock. After execution of $a \in \Actions : \managed(a)=j$, $S_j.\VC(j)$ is incremented by one. 
%
%A shared component is a component which is in the scope of different schedulers. Formally, the set of shared components is defined as
%$B_s=\setof{B_i \mid j,k\in[1,m]: j\neq k \wedge i \in \scope(j) \cap \scope(k) }$.
%
%Awareness of internal action of a shared component $B_{i \in [1,n]} \in B_s$ after execution of the corresponding action $a \in \Actions: \managed(a)=j \wedge i \in \involved(a)$, updates values of $S_k.\VC(j): \scope(k) \cap i \neq \emptyset \wedge i \neq j$ to the value of $S_j.\VC(j)$ at the moment $S_j$ became aware of $\beta_i$.
%
%The way of extending the computation lattice with new nodes is based on finding the happened-before relations between current nodes of the lattice and actions by comparing the vector clocks attached to them. 
%
%Schedulers send their current local vector clocks to the observer along with their state update after execution of each action. 
%
\begin{definition}[Computation lattice]
Computation lattice $\mathcal{L}=(Q \times V,\rightarrowtail)$, where $Q \times V$ is the set of nodes with $Q$ is the set of global states and $V$ is the set of vector clocks.
%
%Formally, computation lattice $\mathcal{L}$ of a distributed system is defined as a tuple of set of nodes (such that each of which is associated to a global state and a unique vector clock) and happened-before relation, $\mathcal{L}=(Q \times V,\rightarrowtail)$, where $Q$ is set of global states and $V$ is set of vector clocks. 
\end{definition}
%
Each node of the lattice is associated to a global state and a unique vector clock.
%
For $\mathcal{L}=(Q \times V,\rightarrowtail)$ and $\eta=(q,\VC) \in Q \times V$, $\eta.clock$ denotes $\VC$ and $\eta.state$ denotes $q$. Set of nodes of the lattice $\mathcal{L}$ is denoted by $\mathcal{L}.nodes$ 
%
\begin{definition}[Happened-before relation]
Happened-before relation is defined between nodes of a computation lattice, $\rightarrowtail\subseteq (Q \times V) \times (Q \times V)$, that is the smallest relation satisfying the following conditions for $a,b,c \in (Q \times V)$ :
\begin{itemize}
	\item if $a.clock > b.clock$, then $a \rightarrowtail b$.
	\item if $a \rightarrowtail b$ and $b \rightarrowtail c$ then $a \rightarrowtail c$.	
\end{itemize}
\end{definition}
%
Two nodes $a$ and $b$ are said to be concurrent if neither $a.clock > b.clock$ nor $b.clock > a.clock$.
% Joint of concurrent nodes $a$ and $b$ is a node $c$ such that $c.clock(i)= \max\left(a.clock(i),b.clock(i)\right)$ for $i \in [1,m]$.
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Making computation lattice}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Reception of a new event either modifies the computation lattice or is kept in a queue to be used later.
%
\begin{definition}[Extensibility]
We define extensibility of lattice $\mathcal{L} = (Q \times V , \rightarrowtail)$ by an event $(a,\VC) \in E_a$ through the function $\ext : Q \times V \times E_a \rightarrow Q \times V$ :
%
%if there exists a node in the lattice $n \in Q \times V$ such that $\exists i \in [1,m], n.clock(i)= \VC(i)-1$ and $\forall j \in [1,m], j \neq i, n.clock(j)= \VC(j)$. 
\begin{itemize}
	\item let $N \subseteq Q \times V$ the set of nodes of the lattice $\mathcal{L}$, that is $N= \mathcal{L}.nodes$,
	\item $\ext(N,(a,\VC)) =\eta$ if $\exists \eta' \in N: \exists i \in [1,m], \eta'.clock(i)= \eta.clock(i)-1 \wedge \forall j \in [1,m], j \neq i, \eta'.clock(j)= \eta.clock(j)$,
	\item $\ext(N,(a,\VC)) = \emptyset$ otherwise.
\end{itemize}
%$\ext(\mathcal{L}.nodes,(a,\VC)) =\eta$ if $\exists \eta' \in \mathcal{L}.nodes: \exists i \in [1,m], \eta'.clock(i)= \eta.clock(i)-1 \wedge \forall j \in [1,m], j \neq i, \eta.clock(j)= \eta.clock(j)$ and  $\ext(\mathcal{L}.nodes,(a,\VC)) = \emptyset$ otherwise. 
%   
%$\ext(\mathcal{L}.nodes,(a,\VC)) =
%   \begin{dcases}
%  \eta  & \text{ if } \exists \eta' \in \mathcal{L}.nodes: \exists i \in [1,m], \eta'.clock(i)= \eta.clock(i)-1 \wedge \forall j \in [1,m], j \neq i, \eta.clock(j)= \eta.clock(j)  \\
%   \emptyset &\text{ otherwise.}
%   \end{dcases}$
where 
$ \eta = ((q_1,\ldots,q_n), \VC), \forall j \in [1,n], q_j=
	\begin{dcases}
   \eta'.state(j)  & j \cap \involved(a)=  \emptyset  \\
   \bot &\text{ otherwise.}
   \end{dcases}$
%

We say lattice $\mathcal{L}$ is extensible by event $e \in E_a$ if $\ext(N,e) \neq \emptyset$.
%
\end{definition}
%
%
%\paragraph{Modified states:}
%For each node $\eta$ created through function $\ext$, we define a function to return the set of indexes of the components which their states have been modified compare to the node that $\eta$ has been extended from. $M(\ext(\mathcal{L}.nodes,(a,\VC)))= \setof{j \mid j \cap \involved(a) \neq \emptyset}$. 
%
\begin{property}
\label{property:ext}
If lattice $\mathcal{L}$ is extensible by an event $(a,\VC)$, then there exists only one node in the lattice in which $\mathcal{L}$ can be extended from by that event.
\end{property} 
%
%We define a FIFO queue $\kappa$ which is a sequence of events.  
%
After reception an event $e\in E_a$ by the observer, if the necessary conditions of extending  the current lattice $\mathcal{L}$ is not satisfied (\ie  $\ext(\mathcal{L}.nodes,e) = \emptyset$), information of event $e$ will be stored in a FIFO queue $\kappa$ for later use.
%
$\kappa$ is initialized with an empty set.
%
\begin{definition}[Nodes update]
We define updating nodes of the lattice $\mathcal{L} = (Q \times V , \rightarrowtail)$ by an event $(\beta_i,q_i) \in E_\beta$ through the function $\upd : Q \times V \times E_\beta \rightarrow Q \times V$. Let $N \subseteq Q \times V$ the set of nodes of the lattice $\mathcal{L}$, that is $N= \mathcal{L}.nodes$,
% 

$\upd(N,(\beta_i,q)) =
	\begin{dcases}
   N  &\text{ if }\exists j \in [1,\length(\kappa)],\kappa(j)=(a,\VC) \wedge i \in \involved(a) \\
   N' &\text{ otherwise.}
   \end{dcases}$

where  $\forall \eta =((q_1,\ldots,q_n),\VC) \in N, \exists! \eta' = (q'_1,\ldots,q'_n),\VC) \in N'$ such that 

$ \forall j \in [1,n], q'_j =
	\begin{dcases}
   q  &\text{ if }q_j=\bot \wedge j=i \\
   q_j &\text{ otherwise.}
   \end{dcases}$
%   
%\begin{itemize}
%	\item $\upd(N,(\beta_i,q)) =N'$ where  $\forall \eta =((q_1,\ldots,q_n),\VC) \in N, \exists! \eta' = (q'_1,\ldots,q'_n),\VC) \in N'$ such that $ \forall j \in [1,n], q'_j =
%	\begin{dcases}
%   q  &\text{ if }q_j=\bot \wedge j=i \\
%   q_j &\text{ otherwise.}
%   \end{dcases}$
%   \item $\upd(N,(\beta_i,q)) = N$ if $\exists (a,\VC) \in \kappa, i \in \involved(a) $
%\end{itemize}
%
\end{definition}
%
After reception an event $e\in E_\beta$ by the observer, if the necessary conditions of updating  the current lattice $\mathcal{L}$ is not satisfied (\ie  $\upd(N,e) = N$), information of event $e$ will be stored in the queue $\kappa$ for later use.
%
In other words, event $e = (\beta_j,q_j)\in E_\beta, j \in [1,n]$ is stored in the queue if there exists an event $e'=(a,\VC) \in E_a$ in the queue such that $e'$ is associated to the execution of an action concerning component $B_j$.
%
\begin{definition}[Queue $\kappa$]
Formally, queue $\kappa=e_1 \cdot e_2 \cdots e_k$ is defined as a sequence over set of events $E_a \cup E_\beta$, \ie $\kappa \in \mathcal{U}$.
\end{definition}
%
%Event $e$, after reception by the observer, is kept in a FIFO queue $\kappa \subseteq E_a \cup E_\beta$ if the necessary conditions for using $e$ in the current lattice $\mathcal{L}$, is not satisfied. $\kappa$ initialized with an empty set.
%
%$\forall e \in  E_a \cup E_\beta , \kappa  = 
%	\begin{dcases}
%   \kappa \cup e  & (e \in E_a \wedge \ext(\mathcal{L}.nodes, e)=  \emptyset) \vee (e=(\beta_j,q_j) \in E_\beta \wedge \exists (a,\VC) \in \kappa, j \in \involved(a)  )  \\
%   \kappa &\text{ otherwise.}
%   \end{dcases}$
%%
%Event $e = (\beta_j,q_j)\in E_\beta, j \in [1,n]$ is kept in the queue if there exists an event $e'=(a,\VC) \in E_a$ in the queue such that $e'$ is associated to the execution of an action concerning component $B_j$. 
%
\begin{definition}[Relation $\mathcal{J}$]
In the lattice $\mathcal{L}=(Q \times V, \rightarrowtail)$, we define relation $\mathcal{J} \subseteq (Q \times V) \times (Q \times V)$ between nodes of the computation lattice. 
%
Two nodes $\eta = ((q_1,\ldots,q_n),(\VC(1),\ldots,\VC(m)))$ and $\eta' = ((q'_1,\ldots,q'_n),(\VC'(1),\ldots,\VC'(m)))$ are in the set of $\mathcal{J}$, that is  $(\eta,\eta') \in \mathcal{J}$, if $\exists! j,k \in [1,m]$ such that $j \neq k$ and $ \VC(j)=\VC'(j)+1 \wedge \VC'(k)=\VC(k)+1 , \forall i\in[1,m], i \neq j \wedge i \neq k, \VC(i)=\VC'(i)$.
%
\end{definition}
%
Intuitively, $\eta$ and $\eta'$ in relation $\mathcal{J}$ are associated to two concurrent events that both could happen from a unique global state of the system which said to be the \textit{meet} of $\eta$ and $\eta'$.
%
\begin{definition}[Meet node]
$\forall \eta,\eta' \in \mathcal{L}.nodes , (\eta,\eta') \in \mathcal{J},  \meet( \setof{\eta,\eta'})=(q'',\VC'') \in \mathcal{L}.nodes , \forall i \in [1,m] : \VC''(i)= \min \setof {\VC(i),\VC'(i)}$.
%
%\begin{property}
%\label{property:joint}
%If $(\eta,\eta') \in \mathcal{J}$ such that $\eta = ((q_1,\ldots,q_n),\VC)$ and $\eta' = ((q'_1,\ldots,q'_n),\VC')$, then $ \forall i \in [1,n], (q_i = q'_i) \vee  (q_i=\bot) \vee (q'_i=\bot)$.
%%
%
%change property to : shared component state are the same in n and n'
%\end{property}
%
\end{definition}
%
\begin{definition}[Joint node]
In the lattice $\mathcal{L}$, if there exists a subset of nodes $N = \setof{\eta^1, \ldots ,\eta^z} \subseteq \mathcal{L}.nodes $ where $\forall i \in [1,z], \eta^i = ((q^i_1,\ldots,q^i_n),(\VC^i(1),\ldots,\VC^i(m)))$, and moreover all nodes in the set $N$ are pairwise in $\mathcal{J}$ relation with the other nodes in the set $N$, that is $\forall n, n' \in N : (n,n') \in \mathcal{J}$, $N$ said to be a \textit{joint set}.
%
For the joint set $N$ there exists a unique meet \ie $\meet(N) \in \mathcal{L}.nodes$.  
%
It is possible to define a joint node $\vartriangle N = ((q_1,\ldots,q_n),(\VC(1),\ldots,\VC(m)))$ where $\forall j \in [1,m], \VC(j) = \max \setof{\VC^i(j) \mid i \in [1,z]}$ and  the state of the joint node is a combination of the latest  modified states of all nodes in the set $N$:

$\forall k \in [1,n], q_k = 
	\begin{dcases}
   q^i_k  &\text{ if } \exists! i \in [1,z] : q^i_k \neq q''_i \\
   q''_i  &\text{ otherwise }(\forall i \in [1,z] : q^i_k = q''_i).
   \end{dcases}$

where  $\meet(N) = ((q''_1,\ldots,q''_n),(\VC''(1),\ldots,\VC''(m)))$.
%
\end{definition}
%
\begin{property}
\label{property:joint}
For a joint set $N$, all the meets of each pairwise nodes in the set $N$ refer to a specific node in the lattice. Therefore $\meet(N)$ is a unique node.
\end{property}
%
%\begin{property}
%\label{property:joint}
%In a joint set $N$, with $N = \setof{\eta^1, \ldots ,\eta^z} $, $\forall i \in [1,z], \eta^i = ((q^i_1,\ldots,q^i_n),(\VC^i(1),\ldots,\VC^i(m)))$:
%%
%%Moreover, for two nodes $\eta^r , \eta^s $ in the joint set such that $M(\eta^r) \cap M(\eta^s) \neq \emptyset$,  $\forall j \in M(\eta^r) \cap M(\eta^s), q^r_j= q^s_j$.
%\begin{itemize}
%	%\item $\forall j \in [1,n]: B_j \in B_s \implies q^1_j = q^2_j = \cdots = q^z_j$. State of a shared components in all nodes in joint set $N$ is similar. 
%	\item $\forall k \in \scope(j):j \in [1,m] \wedge \VC^r(j)=\VC^s(j): r,s \in [1,z] \implies q^r_k = q^s_k$. 
%\end{itemize}
%%
%\end{property}
%
\begin{definition}[Extend by joint nodes]
We define function $\blacktriangle : Q \times V \rightarrow Q \times V$ which takes a set of nodes of a lattice as an input and computes a new set of joint nodes by considering all possible joint sets. 
\begin{itemize}
	\item $\blacktriangle(\emptyset)= \emptyset$
%	\item let $\blacktriangle(N)= N'$
%	\item $\blacktriangle(N \cup \setof{\eta})=   N' \cup \setof{\vartriangle(\eta,\eta') \mid \eta' \in N' \wedge (\eta,\eta') \in \mathcal{J}}  $
	\item $\blacktriangle(N)=  \setof{\vartriangle(N') \not \in N \mid N' \subseteq N \setminus \setof{\setof{\eta} : \eta\in N} \wedge  \forall \eta, \eta' \in N', (\eta, \eta') \in \mathcal{J}}  $
	%\item $\blacktriangle(N)=  \setof{\vartriangle(\eta,\eta') \mid \eta' \in N \wedge (\eta,\eta') \in \mathcal{J}}  $
\end{itemize}
%
Nodes in the set $\blacktriangle(N)$ may be in $\mathcal{J}$ relation with the existing node of the lattice, \ie $N$.
%, or even with themselves.
%
To achieve all the possible joints, we define another function $\joints : Q \times V \rightarrow Q \times V$ which $\joints(N)$ returns the smallest fixed point of function $\blacktriangle$ that is greater or equal than the initial argument $N$. 
\end{definition}
%
\begin{definition}[Recalling events of the queue]
$\recall : Q \times V \times \mathcal{U} \rightarrow Q \times V \times \mathcal{U}$ is defined inductively as follow $\forall i \in [1,j]$ with $j = \length(\kappa)$ 
\begin{itemize}
	\item $\recall (N,\emptyset) =	(N,\emptyset)$,
	\item let $\recall (N,\kappa(i)) =	(N_r,\kappa_r)$,
	\item $\recall (N,\kappa(i+1)) =	
	   \begin{dcases}
   (N',\kappa')  & \text{if } \kappa(i+1) \in E_a \wedge \ext(N_r,\kappa(i+1)) \neq \emptyset \\
   (N'',\kappa')  & \text{if }  \kappa(i+1) \in E_\beta \wedge \upd(N_r,\kappa(i+1)) \neq N\\
   (N_r,\kappa_r) &\text{otherwise.}
   \end{dcases}$
  
where $N'=N_r \cup \ext(N_r,\kappa(i+1)) \cup \joints (N_r \cup \ext(N_r,\kappa(i+1)) )$, $N''=\upd (N_r,\kappa(i+1))$ and $\kappa'=\kappa_r(1) \cdots \kappa_r(i-1) \cdot \epsilon \cdot \kappa_r(i+1)\cdots \kappa_r(j).$
\end{itemize}
\end{definition}
%
%\begin{definition}[Function $\boldsymbol{make}$]
%\label{def:make}
%To show how the set of nodes of the lattice $N$ and a sequence of stored events $\kappa$ (of length $j$) are changed after receiving a new event $e$, we define  function $\make: Q \times V \times \mathcal{U} \times (E_a \cup E_\beta) \longrightarrow Q \times V \times \mathcal{U}$  where:
%%
%\begin{itemize}
%
%	\item $\make(N,\kappa,e) =	
%	   \begin{dcases}
%   (N',\kappa_r)   &  e \in E_a  \wedge \ext(N,e) \neq \emptyset\\
%   (\upd(N,e),\kappa) & e \in E_\beta  \wedge \upd(N,e) \neq N\\
%   (N,\kappa \cdot e) & \text{otherwise.}
%   \end{dcases}$
%   
%where  $N'=N_e \cup N_r$ with $N_e = N \cup \ext(N,e) \cup \joints(N \cup \ext(N,e))$ , $\recall(N_e,\kappa(j))=(N_r,\kappa_r)$.
%
%
%\end{itemize}
%\end{definition}

We define function $\make$ to construct a set of nodes of computation lattice with respect to a sequence of received events.
%
\begin{definition}[Function $\boldsymbol{make}$]
\label{def:make}
Function $\make: \mathcal{U} \longrightarrow Q \times V \times \mathcal{U}$, where:
 
\begin{itemize}
	\item $\make(\epsilon)=( \mathcal{L}_\init, \emptyset )=( (\init , (0,\ldots,0)), \emptyset )$,
	\item let $\make(u)= ( N, \kappa ) $
	\item $\make(u \cdot e) =	
	   \begin{dcases}
   (N',\kappa_r)   &  e \in E_a  \wedge \ext(N,e) \neq \emptyset\\
   (\upd(N,e),\kappa) & e \in E_\beta  \wedge \upd(N,e) \neq N\\
   (N,\kappa \cdot e) & \text{otherwise.}
   \end{dcases}$
   
where  $N'=N_e \cup N_r$ with $N_e = N \cup \ext(N,e) \cup \joints(N \cup \ext(N,e))$ , $\recall(N_e,\kappa(j))=(N_r,\kappa_r)$ and  $j = \length(\kappa)$.
%	\item $\make(u \cdot (a,\VC)) =	
%	   \begin{dcases}
%   N' \cup \joints(N')   &  \ext(\make(u),(a,\VC)) \neq \emptyset\\
%   \make(u) &\text{otherwise.}
%   \end{dcases}$
%   
%where  $N' = N \cup \ext(\make(u),(a,\VC)) \in Q \times V$ 
%	\item $\make(u \cdot (\beta_j,q_j)) =	
%	   \begin{dcases}
%   \make(u)  &  \exists (a,\VC) \in \kappa \wedge j \in \involved(a)\\
%   \upd(\make(u),(\beta_j,q_j)) &\text{otherwise.}
%   \end{dcases}$
%   
%   $\forall \eta = ((q'_1,\ldots,q'_n),\VC) \in N, \exists! \eta'= ((q''_1,\ldots,q''_n),\VC) \in N' , q''_j=
%	\begin{dcases}
%   q_j  &\text{ if }q'_j=\bot \\
%   q'_j &\text{ otherwise.}
%   \end{dcases}$
%
\end{itemize}
\end{definition}
%
%We define function $\make$ to construct a computation lattice with respect to a sequence of received events.
%%
%\begin{definition}[Function $\boldsymbol{make}$]
%\label{def:make}
%Function $\make: \mathcal{U} \longrightarrow \mathcal{L}$, where:
% 
%\begin{itemize}
%	\item $\make(\epsilon)=\mathcal{L}_\init=(\init , (0,\ldots,0))$,
%	\item let $\make(u)= (N , \rightarrowtail)$, where $N \in Q \times V,$
%	\item $\make(u \cdot (a,\VC)) =	
%	   \begin{dcases}
%  ( N' \cup \joints(N') , \rightarrowtail')  &  \ext(\make(u),(a,\VC)) \neq \emptyset\\
%   \make(u) &\text{otherwise.}
%   \end{dcases}$
%   
%where  $N' = N \cup \ext(\make(u),(a,\VC)) \in Q \times V$ 
%	\item $\make(u \cdot (\beta_j,q_j)) =	
%	   \begin{dcases}
%   \make(u)  &  \exists (a,\VC) \in \kappa \wedge j \in \involved(a)\\
%   ( N', \rightarrowtail) &\text{otherwise.}
%   \end{dcases}$
%   
%   $\forall n = ((q'_1,\ldots,q'_n),\VC) \in N, \exists! n'= ((q''_1,\ldots,q''_n),\VC) \in N' , q''_j=
%	\begin{dcases}
%   q_j  &\text{ if }q'_j=\bot \\
%   q'_j &\text{ otherwise.}
%   \end{dcases}$
%%
%\end{itemize}
%\end{definition}
%$\mathcal{L}$  is initially consists of a node $\mathcal{L}_\init=(\init , (0,\ldots,0))$.
%
\begin{proposition}
\label{proposition:make}
$\forall u , u' \in \mathcal{U}: u = u_1 \cdot u_2 \cdot u_3 \cdots u_i ,  u' = u'_1 \cdot u'_2 \cdot u'_3 \cdots u'_j$

$(i=j) \wedge \setof{u_1 , u_2 , u_3, \ldots ,u_i}=\setof{u'_1 , u'_2 , u'_3 ,\ldots ,u'_j} \implies \make(u)=\make(u')$.
\end{proposition}
%
Proposition~\ref{proposition:make} states that changing the reception order of the events does not affect the output result of the function $\make$.
%
%\paragraph{Define a function to make lattice:}
%We define function $make : \mathcal{U} \rightarrow \mathcal{L}$ to make a computation lattice with respect to a sequence of received events.
%%
%$\mathcal{L}$  is initially consists of a node $\mathcal{L}_\init=(\init , 0)$ where $0$ represents a vector clock with all element of zero.
%%
%Function $make$ uses three following algorithms according to the type of received event. 
%
%\begin{itemize}
%	\item if $make(u \cdot (a,\VC))= make(u).(Q \times V) \cup ((q'_1,\ldots,q'_n),\VC))$ where $\forall j \in [1,n], q'_j=
%	\begin{dcases}
%   q_j  & j \cap \involved(a)=  \emptyset  \\
%   \bot &\text{ otherwise.}
%   \end{dcases}$
%\end{itemize}
%\paragraph{Extending:}
%Event $e=(a,(\VC(1),\ldots,\VC(m)))$ can extend lattice $\mathcal{L}$ if there exists a node $n$ in the lattice such that $n=((q_1,\ldots,q_n),(\VC'(1),\ldots,\VC'(m)))$ and $\exists! i\in [1,m], \VC(i)=\VC'(i)+1$. The new node $n'$ is defined as $((q'_1,\ldots,q'_n),(\VC(1),\ldots,\VC(m)))$ where $\forall j \in [1,n], q'_j=
%	\begin{dcases}
%   q_j  & j \cap \involved(a)=  \emptyset  \\
%   \bot &\text{ otherwise.}
%   \end{dcases}$
%We say lattice $\mathcal{L}$ is extendable by event $e$.
%%
%Event $e$ is kept in a FIFO queue if the prerequisite of extension of  lattice $\mathcal{L}$ is not satisfied.
%
%
%\paragraph{Making joints of two nodes:}
%Considering two nodes $n=((q_1,\ldots,q_n),(\VC(1),\ldots,\VC(m)))$ and $n'=((q'_1,\ldots,q'_n),(\VC'(1),\ldots,\VC'(m)))$ such that $\exists! j,k \in [1,m], j \neq k, \VC(j)=\VC'(j)+1 \wedge \VC'(k)=\VC(k)+1 , \forall i\in[1,m], i \neq j \wedge i \neq k, \VC'(i)=\VC(i) \wedge \forall z \in [1,n], (q_z = q'_z) \vee  (q_z=\bot) \vee (q'_z=\bot) $, a joint node $n''=((q''_1,\ldots,q''_n),(\VC''(1),\ldots,\VC''(m)))$ is a possible node in the computation lattice such that $\forall i \in [1,m], \VC''(i) = \max (\VC(i),\VC'(i))$ and $\forall j \in [1,n], q''_j=
%	\begin{dcases}
%   \bot  & (q_j=\bot) \vee (q'_j=\bot) \\
%   q_j &\text{ otherwise.}
%   \end{dcases}$
%%
%
%After extending the lattice and making possible joints, events stored in the queue must be recalled in order to check if they could be applied in the new lattice configuration.  
%
%\paragraph{Updating:}
%After receiving event $e=(\beta_j,q_j), j \in [1,n]$, each node of the lattice, that it $((q'_1,\ldots, q'_j, \ldots ,q'_n),\VC)$, is updated to $((q'_1,\ldots, q_j, \ldots ,q'_n),\VC)$ if $q'_j \in Q^b_j$. 
%%
%Event $e$ is kept in the queue if there exists an event $e'=(a,\VC)$ in the queue such that $j \cap \involved(a) \neq \emptyset$.
%
%
%\begin{proposition}
%$\forall u , u' \in \mathcal{U}: u = u_1 \cdot u_2 \cdot u_3 \cdots u_i ,  u' = u'_1 \cdot u'_2 \cdot u'_3 \cdots u'_j$
%
%$i=j \wedge \setof{u_1 , u_2 , u_3, \ldots ,u_i}=\setof{u'_1 , u'_2 , u'_3 ,\ldots ,u'_j} \implies make(u)=make(u')$.
%\end{proposition}
%
%Observer computes possible joint nodes.
%%
%For instance, after receiving two state updates with the vector clock of $(0,1)$ and $(1,0)$, a new node with vector clock of $(1,1)$ is automatically generated.  
%
%\paragraph{happened-before relation:}
%The relation between nodes of the lattice $\rightarrowtail\subseteq (Q \times V) \times (Q \times V)$ is the smallest relation satisfying the following conditions for $a,b,c \in (Q \times V)$ :
%\begin{itemize}
%	\item if $a=(q_a,\VC_a)$ , $b=(q_b,\VC_b)$ and $\VC_a > \VC_b$, then $a \rightarrowtail b$.
%
%	%\item if $\managed(a) = \managed(b)$, and $a$ comes before $b$, then $a \rightarrowtail b$.
%	%\item if $\managed(a) \neq \managed(b)$, then $a \rightarrowtail b$ and $b \rightarrowtail a$ are two possible relations between $a$ and $b$, unless $\involved(a) \cap \involved(b) \neq \emptyset$ which in this case only one one those possible relation is valid.
%	%\item If scheduler $S_{j \in [1,m]}$ executes an action $a \in \Actions$ with a shared component $B_{i \in [1,n]} \in B_s$, $i \in \involved(a)$, all actions in scheduler $S_j$ before awareness of internal action of $B_i$ are happened before all actions of schedulers in the set $\setof{S_k \mid i \in \scope(k)}$ after awareness of internal action of $B_i$.
%	\item if $a \rightarrowtail b$ and $b \rightarrowtail c$ then $a \rightarrowtail c$.	
%\end{itemize}
%%
%Two nodes $a$ and $b$ are said to be concurrent if neither $\VC_a > \VC_b$ nor $\VC_b > \VC_a$. Joint of concurrent nodes $a$ and $b$ is a node $c$ such that $\VC_c(i)= \max\left(\VC_a(i),\VC_b(i)\right)$ for $i \in [1,m]$. 
%
%\begin{property}
%\label{prop:virtualmessage}
%If scheduler $S_{j \in [1,m]}$ executes an action $a \in \Actions$ with a shared component $B_{i \in [1,n]} \in B_s$, $i \in \involved(a)$, all actions in scheduler $S_j$ before awareness of internal action of $B_i$ are happened before all actions of schedulers in the set $\setof{S_k \mid i \in \scope(k)}$ after awareness of internal action of $B_i$.
%%An internal action of a shared component $B_{i \in [1,n]} \in B_s$ in the scheduler $S_{j \in [1,m]}$ which did the last action concerned component $B_i$, can be seen as set of virtual send messages form $S_j$ to the other schedulers which have component $B$ in their scope. These virtual messages are received ideally to the destinations with no time delay.
%\end{property}
\input{lattice}
%
\begin{example}
\figref{fig:lattice} depicts the computation lattice according to the local traces of Example~\ref{xmp:dmodel}. 
%
%
Three paths from the initial node $\left( \left( d_1,d_2,d_3 \right),\left( 0,0 \right) \right)$ to the last node $\left( \left( f_1,\bot,\bot \right),\left( 1,2 \right) \right)$, show all three possible global traces.
%
Nodes $\left( \left( d_1,d_2,f_3 \right),\left( 0,1 \right) \right)$ associated to the action $f_{12}$ and $\left( \left( f_1,f_2,d_3 \right),\left( 1,0 \right) \right)$ associated to the action $f_3$ are concurrent which is the cause of generation of joint node $\left( \left( f_1,f_2,f_3 \right),\left( 1,1 \right) \right)$.
% whereas $f_{12}$ and $d_{23}$ due to being involved with the shared component $B_2$ are related together such that $f_{12} \rightarrowtail d_{23}$.
Due to vector clock update technique, the node with vector clock of $(0,2)$ does not exist.
\end{example}
%
\begin{definition}[Set of paths]
$\mathcal{N} = \setof{\eta_0 \cdot \eta_1 \cdot \eta_2 \cdots \eta_i\mid \eta_0 = \mathcal{L}_\init , \forall j \in [0,i-1],n_j \rightarrowtail \eta_{j+1}}$ is the set of paths of the computation lattice $\mathcal{L}$.
%
Each path is defined as a sequence of nodes of the lattice.  
\end{definition} 
%
Each path of computation lattice represents a possible global trace of system.
%
\begin{definition}[Global trace]
The sequence $\sigma = q_0 \cdot q_1 \cdot q_2 \cdots q_i$ represents the corresponding trace of the path  $\eta_0 \cdot n_1 \cdot \eta_2 \cdots \eta_i$ in the lattice $\mathcal{L}$ such that $\forall j \in [0,i], q_j = \eta_j . state$.
%
\end{definition} 
%
%



==> lattice-making.tex <==
%\algnewcommand\algorithmicinput{\textbf{Global variables:}}
%\algnewcommand\INPUT{\item[\algorithmicinput]}
%\begin{algorithm}
%\caption{$\make$}
%\label{alg:make}
%\begin{algorithmic}[1]
%%\INPUT{$\mathcal{L},\kappa, V$}
%\INPUT{$\mathcal{L}$ initialized to $\init_{\mathcal{L}}$,
%
%$\qquad \qquad \ \kappa$ initialized to an empty sequence,
%
%$\qquad \qquad \ V$ initialized to $(0,\ldots,0)$ elements.}
%%\INPUT{$\kappa$ initialized to an empty sequence}
%%\INPUT{$V$ initialized to an empty sequence}
%\Procedure{Make}{$e, \fromthequeue$}
%\If {$e \in E_{\rm a}$} \label{line:start_action_event}
%\Comment{if $e$ is an action event.}
%	\State $\textsc{ActionEvent}	(e,\fromthequeue)$
%\ElsIf {$e \in E_{\upbeta}$} \label{line:start_update_event}
%\Comment{if $e$ is an update event.}
%	\State $\textsc{UpdateEvent}	(e,\fromthequeue)$
%\EndIf \label{line:end_update_event}
%\EndProcedure
%%
%\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}
%\caption{\textsc{ActionEvent}}
%\begin{algorithmic}[1]
%%
%\Procedure{ActionEvent}{$e, \fromthequeue$}
%\State{$\latticextend \gets \false$}
%\For {all $\eta \in \mathcal{L}.\mathit{nodes}$}	
%		\If {$\exists \eta' : \eta' = \upda(\eta,e)$}
%			\State { $\mathcal{L}.nodes \gets \mathcal{L}.\mathit{nodes} \cup  \eta'$}
%			\Comment{extend the lattice with the new node.}
%			\State $\textsc{ModifyQueue}(e,\fromthequeue,\true)$
%			\Comment{event $e$ is removed from the queue if it was picked up from the queue.}
%			\State{$\latticextend \gets \true$}
%			\State {\textbf{break}}
%			\Comment{stop iteration  when the lattice is extended (Property~\ref{property:ext}).}
%		\EndIf
%	\EndFor
%	\If {$\neg \latticextend$}
%%		\State {$\kappa \gets \kappa \cdot e$}
%%		\Comment{event $e$ is added to the queue if it can't extend the lattice.}
%		\State $\textsc{ModifyQueue}(e,\fromthequeue,\false)$
%		\Comment{event $e$ is added to the queue if it was not picked up from the queue.}
%		\State {\textbf{return}}
%	\EndIf
%	\State $\textsc{Joints(~)}$ \label{line:make_joints}
%	\Comment{extend the lattice by joint nodes.}
%	\State $\textsc{UpdateV}\textsc{(}e\textsc{)}$ \label{line:global_variables_update}
%	\Comment{update global variables based on action event $e$.}
%	\If {$\neg \fromthequeue$}
%		\State $\textsc{CheckQueue(~)}	$ \label{line:check_queue}
%		\Comment{recall the events stored in the queue.}
%%	\Else 
%%		\State {\textbf{return}}
%%		\label{line:return_if_from_queue}
%%		\Comment{return if event $e$ can not extend the lattice.}	
%	\EndIf
%\EndProcedure
%%
%\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}
%\caption{\textsc{UpdateEvent}}
%\begin{algorithmic}[1]
%%
%\Procedure{UpdateEvent}{$e, \fromthequeue$}
%	\For {all $e' \in \kappa  $}	
%		\If {$e' \in E_{\rm a} \wedge e.\mathit{index} \in \involved(e'.\mathit{action})$}
%		\Comment{check if there exists an action event in the queue concerning component $B_{e.\mathit{index}}$.}
%		\State $\textsc{ModifyQueue}	(e,\fromthequeue,\false)$
%		\Comment{event $e$ is added to the queue if it was not picked up from the queue.}
%%			\State {$\kappa \gets \kappa \cdot e$}
%%			\Comment{event is added to the queue if the update condition does not hold.}
%			\State {\textbf{return}}			
%		\EndIf
%	\EndFor
%	\If {$B_{e.index} \in B_{\rm s}$} 
%		%\State {$e.\mathit{clock} \gets \vc_{e.\mathit{sender}}^{e.\mathit{index}}$}
%	\Comment{if the event is associated to a shared component.}
%	\State $\textsc{SharedComponentEvent}	(e)$
%	\label{line:shared_component_event}
%	\Else 
%	\For {all $\eta \in \mathcal{L}.\mathit{nodes}$}	\label{line:start_update_nodes}
%		\State {$\eta \gets \updb(\eta,e)$}
%		\Comment {update nodes according to Definition~\ref{def:node_update}.}
%	\EndFor		\label{line:end_update_nodes}
%	\EndIf
%	\State $\textsc{ModifyQueue}	(e,\fromthequeue,\true)$
%\EndProcedure
%%
%\end{algorithmic}
%\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%			
%\algstore{myalg}
%\end{algorithmic}
%\end{algorithm}
%%\clearpage
%\begin{algorithm}
%\ContinuedFloat
%\caption{$\make$ (continued)}
%\begin{algorithmic}
%\algrestore{myalg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{algorithm}
%\caption{\textsc{Jcompute}}
%\begin{algorithmic}[1]
%%
%\Procedure{Jcompute}{}
%		\For {all $\eta,\eta',\eta'' \in\mathcal{L}.\mathit{nodes}$}	
%			\If {$\eta''\rightarrowtail \eta \wedge \eta''\rightarrowtail \eta'$} 	
%			\Comment{if $\eta$ and $\eta'$ are associated to two concurrent events.}		
%				\State {$\mathcal{J}_{\mathcal{L}}=\mathcal{J}_{\mathcal{L}} \cup \setof{(\eta.\mathit{clock},\eta'.\mathit{clock})}$}
%				\Comment{$\eta.\mathit{clock}$ and $\eta'.\mathit{clock}$ are added to relation $\mathcal{J}_{\mathcal{L}}$.}
%			\EndIf
%		\EndFor 
%		\State {\textbf{return} $\mathcal{J}_{\mathcal{L}}$}  
%\EndProcedure
%%
%\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}
%\caption{\textsc{Joints}}
%\begin{algorithmic}[1]
%%
%%
%\Procedure{Joints}{}
%    \State $\mathcal{J}_{\mathcal{L}}\gets\textsc{Jcompute}$       
%	\Comment{compute the pairs of the vector clocks of the nodes which are in $\mathcal{J}_{\mathcal{L}}$.}
%	\While {$\mathcal{J}_{\mathcal{L}} \neq \emptyset$ }
%		\For {all $\eta,\eta' \in\mathcal{L}.\mathit{nodes} \wedge (\eta.\mathit{clock},\eta'.\mathit{clock}) \in \mathcal{J}_{\mathcal{L}}$}	
%		\State {$\mathcal{L}.\mathit{nodes} \gets \mathcal{L}.\mathit{nodes} \cup \setof{\joint(\eta,\eta',\mathcal{L})}$}
%		\Comment{extend the lattice with the new joint node.}
%		\State {$\mathcal{J}_{\mathcal{L}} \gets \mathcal{J}_{\mathcal{L}} \setminus \{(\eta.\mathit{clock},\eta'.\mathit{clock})\}$}
%		\EndFor
%   		\State $\mathcal{J}_{\mathcal{L}}\gets\textsc{Jcompute}$       
%	\EndWhile	
%	%\State \textbf{return} $\mathcal{L}$
%\EndProcedure
%%
%%
%\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}
%\caption{\textsc{CheckQueue}}
%\begin{algorithmic}[1]
%%
%%
%\Procedure{CheckQueue}{}
%%	\State $\textsc{ModifyQueue}	(e,\kappa,\fromthequeue,\false)$
%	\While {$\true $ } \label{line:while_update}
%		\State {$\kappa' \gets \kappa$}
%		\label{line:queue_copy}
%		\For {all $z\in [1,\length(\kappa)]$}	
%			\State {$\make(\kappa(z),\true)$}
%			\Comment{recall the events of the queue.}
%		\EndFor 
%		%\State {$\fromthequeue \gets \false$}
%		\If {$\kappa=\kappa'$} \label{line:start_check_equality}
%			\State {\textbf{break}}	\label{line:break}		
%			\Comment{break if none of the events in the queue is used.}
%		\EndIf \label{line:end_check_equality}
%	\EndWhile 
%\EndProcedure
%%
%%
%\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}
%\caption{\textsc{SharedComponentEvent}}
%\begin{algorithmic}[1]
%%
%%
%\Procedure{SharedComponentEvent}{$e$}
%    \For {all $\eta \in \mathcal{L}.\mathit{nodes}$}	\label{line:start_update_nodes_shared}
%			%\If {$\eta.\mathit{clock} \geq e.\mathit{clock}$}
%			\If {$\eta.\mathit{clock} \geq \vc_{e.\mathit{sender}}^{e.\mathit{index}}$} \label{line:vc1}
%				\State {$updatable \gets \true$}
%					\For {all $j\in [1,m]\setminus \{e.\mathit{sender}\} \wedge e.\mathit{index} \in \scope(j)$}
%							\If {$\eta.\mathit{clock} \geq  \vc_j^{e.\mathit{index}}$} \label{line:vc2}
%								\State {$updatable \gets \false$}
%								\State {\textbf{break}}
%							\EndIf
%					\EndFor
%			\EndIf
%			\If {$updatable$}
%				\State {$\eta \gets \updb(\eta,e)$} \label{line:updatable}
%			\EndIf
%		\EndFor \label{line:end_update_nodes_shared}
%\EndProcedure
%%
%\end{algorithmic}
%\end{algorithm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%			
%\algstore{myalg}
%\end{algorithmic}
%\end{algorithm}
%%\clearpage
%\begin{algorithm}
%\ContinuedFloat
%\caption{$\make$ (continued)}
%\begin{algorithmic}
%\algrestore{myalg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{algorithm}
%\caption{\textsc{ModifyQueue}}
%\begin{algorithmic}[1]
%%
%\Procedure{ModifyQueue}{$e,\fromthequeue,\eventused$}
%			\If {$\fromthequeue \wedge \eventused$}
%				\State {$\kappa \gets \rem(\kappa,e)$}
%				\label{line:remove_queue}
%				\Comment{event $e$ is removed from the queue if it is picked from queue and used.}
%			\ElsIf {$\neg \fromthequeue \wedge \neg \eventused$}
%				\State {$\kappa \gets \kappa \cdot e$}
%				\label{line:add_queue}
%				\Comment{event $e$ is added to the queue if it is not picked from queue and could not be used.}
%			\EndIf
%\EndProcedure
%%
%%
%\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}
%\caption{\textsc{UpdateV}}
%\begin{algorithmic}[1]
%%
%%
%\Procedure{UpdateV}{$e$}
%	\State{$j \gets \managed(e).\mathit{index}$} \label{line:start_last_vc}
%	\For {all $i \in \{i \in [1,n] \mid  B_i\in B_{\rm {s}} \wedge i \in \scope(j) \wedge i \in \involved(e.\mathit{action})\}$}	
%		\State {$\vc_j^i \gets e.\mathit{clock}$}
%		\Comment{store the vector clock in the dedicated variable.}
%		\label{line:last_vc}
%	\EndFor \label{line:end_last_vc}
%\EndProcedure
%%
%\end{algorithmic}
%%
%\end{algorithm}
%
%

==> rvltl.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{LTL Runtime Verification by Progression on the Reconstructed Computation Lattice}
\label{sec:ltl}
%%%%%%%%%%%%%%%%%%%%%%
%

In this section, we address the problem of monitoring an LTL formula specifying the desired global behavior of the system.

In the usual case, evaluating whether an LTL formula holds requires the monitoring procedure to have access to the complete information about the system state, that is ready states of CBSs.
%
Since components have busy states as well as ready states, the global trace of the system is a sequence of incomplete global states (\cf \defref{def:global-trace}).
%
An incomplete global state is a sort of global state in which the state of some components are possibly unknown.
%
Although by stabilizing the system to have all the components' ready-states we could obtain a complete  computation lattice using algorithm $\make$ (\cf \secref{subsec:algorithm}), that is the state of each node is a complete global state, instead, we propose an on-the-fly verification of an LTL property during the construction of computation lattice.
%


There are many approaches to monitor LTL formulas based on various finite-trace semantics (\cf~\cite{bauer10}).
%
One way of looking at the monitoring problem for some LTL formula $\varphi$ is described in~\cite{bauer12} based on formula rewriting, which is also known as formula progression, or just \textit{progression}.
%
Progression splits a formula into (i) a formula expressing what needs to be satisfied by the observed events so far and (ii) a new formula (referred to a \textit{future goal}), which has to be satisfied by the trace in the future.
%
We apply progression over a set of finite traces, where each trace consists in a sequence of (possibly) incomplete global states, encoded from the constructed computation lattice. 
%
An important advantage of this technique is that it often detects when a formula is violated or validated before the end of the execution trace, that is, when the constructed lattice is not complete, so it is suitable for online monitoring.

To monitor the execution of a distributed CBS with multi-party interaction with respect to an LTL property $\varphi$, we introduce a more informative computation lattice by attaching to the each node of lattice $\mathcal{L}$ a set of formula.
%
Given a computation lattice $\mathcal{L} = \left( N,\xrightarrowtail[] \right)$ (as per \defref{def:computation_lattice}), we define 
an augmented computation lattice $\mathcal{L}^\varphi$ as follow.
%
\begin{definition}[Computation lattice augmentation]
$\mathcal{L}^\varphi$ is a pair  $\left( N^\varphi ,\xrightarrowtail[] \right)$, where $N^\varphi \subseteq Q^l \times \VC \times 2^{\LTL}$ is the set of nodes augmented by $2^{\LTL}$, that is the set of LTL formulas.
%
The initial node is $\init^{\varphi}_{\mathcal{L}}= (\init,(0,\ldots,0),\{\varphi\})$ with $\varphi \in \LTL$  the global desired property. 
%
\end{definition}
%
In the newly defined computation lattice, a set of LTL formulas is attached to each node. 
%
The set of formulas attached to a node represents the different evaluation of the property $\varphi$ with respect to different possible paths form the initial node to the node.
%
The state and the vector clock associated to each node and the happened-before relation are defined similar to the initial definition of computation lattice (\cf \defref{def:computation_lattice}).
%

The construction of the augmented computation lattice requires some modifications to algorithm $\make$:
%
\begin{itemize}
	\item Lattice $\mathcal{L}^\varphi$ initially has node $\init^{\varphi}_{\mathcal{L}}= (\init,(0,\ldots,0),\{\varphi\})$.
	\item The creation of a new node $\eta$ in the lattice with $\eta.\mathit{state}=q$ and $\eta.\mathit{clock}=\vc$, calculates the set of formulas $\Sigma$ associated to $\eta$ using the progression function (see \defref{def:progression}).
	The augmented node is $\eta= ( q, \vc, \Sigma )$, where $\Sigma = \{ \prog(\LTL',q) \mid   \LTL' \in \eta'.\Sigma \wedge ( \eta' \xrightarrowtail[] \eta \vee \exists N \subseteq \mathcal{L}^\varphi.\mathit{nodes} : \eta'=\meet(N,\mathcal{L}) \wedge \eta =\joint(N,\mathcal{L}) )\}$.
	%
	We denote the set of formulas of node $\eta \in \mathcal{L}^\varphi.\mathit{nodes}$ by $\eta.\Sigma$.
	%
%	The set of formulas represents the different evaluation of the property $\varphi$ with respect to different possible paths form the initial node to node $\eta$.
	%
	\item Updating node $\eta=( q, \vc, \Sigma )$ by   update event $e = (\beta_i,q_i)\in E_\upbeta, i\in [1,n]$ which is sent by scheduler $S_j, j\in[1,m]$ updates all associated formulas $\Sigma$ to $\Sigma'$ using the update function (see \defref{def:update}), where
%
$\Sigma' = \setof{ \updfct_\varphi (\LTL,q_i,j) \mid \LTL \in \Sigma }$.
\end{itemize} 
%
\begin{definition}[Progression function]
\label{def:progression}
$\prog: \LTL \times Q^l \longrightarrow \LTL $ is defined using a pattern-matching with $p\in AP_{i\in[1,n]}$ and $q=(q_1,\dots,q_n)\in Q^l$.
%
\[
\begin{array}{rcl}
 \prog(\varphi, q )  & = & \mathtt{match} (\varphi) \;\mathtt{with}\\
        & \mid &  p\in AP_{i\in[1,n]} \rightarrow \begin{dcases}   
T &\text{ if } q_i \in Q^{\rm r}_i \wedge p\in q_i \\
F &\text{ if } q_i \in Q^{\rm r}_i \wedge p\not\in q_i\\
\textbf{X}^k_\beta p  &\text{ otherwise }(q_i = \bot^k_i, k \in[1,m])\\
   \end{dcases} \\
        & \mid &  \textbf{X}^k_\beta p \rightarrow 
        \textbf{X}^k_\beta p\\
        & \mid &  \varphi_1 \vee \varphi_2 \rightarrow \prog(\varphi_1, q)\vee \prog(\varphi_2,q)\\
        & \mid &  \varphi_1 \textbf{U} \varphi_2 \rightarrow \prog(\varphi_2, q)\vee \prog(\varphi_1,q) \wedge \varphi_1 \textbf{U} \varphi_2\\        
		& \mid &  \textbf{G} \varphi \rightarrow \prog(\varphi, q)\wedge \textbf{G}\varphi\\		
		& \mid & \textbf{F} \varphi \rightarrow \prog(\varphi, q)\vee \textbf{F}\varphi\\		
		& \mid &  \textbf{X} \varphi \rightarrow \varphi\\		
		& \mid &  \neg \varphi \rightarrow \neg \prog(\varphi, q)\\	
        & \mid &  T \rightarrow T
\end{array}
\]
%
We define a new modality $\textbf{X}_\beta$ such that $\textbf{X}^k_\beta p$ for $p\in AP_{i\in[1,n]}$ and $k \in[1,m]$ means that atomic proposition $p$ has to hold at next ready state of component $B_i$ which is sent by scheduler $S_k$.
%
For a sequence of global states obtained at runtime $ \sigma=q_0\cdot q_1 \cdot q_2 \cdots$ such that  $\sigma_j=q_j $, we have  $\sigma_j \models \textbf{X}^k_\beta p \Leftrightarrow \sigma_z \models p$ where\\  $z=\min\left(\setof{r>j \lmid \left( \sigma_{r-1}\downarrow_{S_k} \right) \goesto[\beta_i]_{S_k} \left( \sigma_r\downarrow_{S_k} \right) } \right)$.
\end{definition}
%
The truth value of the progression of an atomic proposition $p\in AP_i$ for $i \in [1,n]$ with a global state  $q=(q_1,\dots,q_n)$ is evaluated by true (\resp false) if the state of component $B_i$ (that is $q_i$) is a ready state and satisfies (\resp does not satisfy) the atomic proposition $p$.
%
If the state of component $B_i$ is not a ready state, the evaluation of the atomic proposition $p$ is postponed to the next ready state of component $B_i$.
%
\begin{definition}[Formula update function]
\label{def:update}
$\updfct_\varphi: \LTL \times \setof{Q^{\rm r}_i}^n_{i=1}  \times [1,m] \rightarrow \LTL$ is defined using a pattern-matching with $q_i \in Q^{\rm r}_i$ for $i \in [1,n]$.
%
\[
\begin{array}{rcl}
 \updfct_\varphi(\varphi, q_i, j)  & = & \mathtt{match} (\varphi) \;\mathtt{with}\\
        & \mid &  \textbf{X}^k_\beta p \rightarrow \begin{dcases}
T & \text{ if }  p \in \AP_i \cap q_i \wedge k=j\\
F & \text{ if }  p\in \AP_i \cap \overline{q_i} \wedge k=j\\
\textbf{X}^k_\beta p &\text{ otherwise } (p\not\in AP_i \vee k\neq j)
   \end{dcases} \\
        & \mid &  \varphi_1 \vee \varphi_2 \rightarrow \updfct_\varphi(\varphi_1,q_i)\vee \updfct_\varphi(\varphi_2,q_i)\\
        & \mid &  \varphi_1 \wedge\varphi_2 \rightarrow \updfct_\varphi(\varphi_1,q_i)\wedge \updfct_\varphi(\varphi_2,q_i)\\        
        & \mid & \varphi_1 \textbf{U} \varphi_2 \rightarrow \updfct_\varphi(\varphi_1, q_i) \textbf{U} \updfct_\varphi(\varphi_2,q_i)\\                
		& \mid &  \textbf{G} \varphi \rightarrow \textbf{G} \updfct_\varphi(\varphi, q_i)\\				
		& \mid & \textbf{F} \varphi \rightarrow \textbf{F}\updfct_\varphi(\varphi, q_i)\\				
		& \mid &  \textbf{X} \varphi \rightarrow \textbf{X}\updfct_\varphi(\varphi, q_i)\\				
		& \mid &  \neg \varphi \rightarrow  \neg \updfct_\varphi(\varphi ,q_i)\\	
        & \mid &  T \rightarrow T\\
        & \mid &  p\in AP_{ i \in[1,n] } \rightarrow p
\end{array}
\]
%
\end{definition}
%
Update function updates a progressed LTL formula with respect to a ready state of a component.
%
Intuitively, a formula consists in an atomic proposition  whose truth or falsity depends on the next ready state of component $B_i$ sent by scheduler $S_k$, that is  $\textbf{X}^k_\beta p$ where $p\in \AP_i$, can be evaluated using update function by taking the first ready state of component $B_i$ received from scheduler $S_k$ after the formula rewrote to $\textbf{X}^k_\beta p$.
%
\input{table}
%
\begin{example}[Formula progression and formula update over an augmented computation lattice] 
Let consider the system in \exref{xmp:dmodel} with global trace $t_2$ and the received sequence of events presented in \exref{xmp:seqevents} and desired property $\varphi = \textbf{G} (d_3 \vee f_1)$.
%
$\mathcal{L}^\varphi$ initially has node $\init^{\varphi}_{\mathcal{L}}= ((d_1,d_2,d_3),(0,0),\{\varphi\})$.
%
By observing the action event $(\fil_{12},(1,0))$, algorithm $\make$ creates new node $\eta_1 = ((\bot, \bot, d_3),(1,0), \setof{\varphi })$, because 
%
$\prog(\textbf{G} (d_3 \vee f_1),(\bot, \bot,d_3))=\prog((d_3 \vee f_1),(\bot, \bot,d_3)) \wedge \textbf{G} (d_3 \vee f_1) = T \wedge \textbf{G} (d_3 \vee f_1) = \textbf{G} (d_3 \vee f_1) = \varphi$.

%
By observing the action event $(\fil_3,(0,1))$, new node $\eta_2 = ((d_1, d_2, \bot),(0,1), \setof{\textbf{X}_\beta d_3 \wedge \varphi })$ is created, because
%
$\prog(\textbf{G} (d_3 \vee f_1),(d_1, d_2,\bot))=\prog((d_3 \vee f_1),(d_1, d_2,\bot)) \wedge \textbf{G} (d_3 \vee f_1) = \textbf{X}_\beta d_3 \wedge \textbf{G} (d_3 \vee f_1)= \textbf{X}_\beta d_3 \wedge \varphi $.
%
Formula $\textbf{X}_\beta d_3$ means that the evaluation of incomplete state $(d_1, d_2,\bot)$ with respect to formula $(d_3 \vee f_1)$ is on hold until the next ready state of component $\tank_3$.

%
Consequently joint node 
$\eta_3 = ((\bot, \bot, \bot),(1,1), \{ (\textbf{X}_\beta d_3) \wedge (\textbf{X}_\beta d_3 \vee \textbf{X}_\beta f_1)  \wedge \varphi, (\textbf{X}_\beta d_3 \vee \textbf{X}_\beta f_1)\wedge \varphi, (\textbf{X}_\beta d_3 \vee \textbf{X}_\beta f_1)\wedge \varphi\})$ is made.
%
The update event $(\beta_3,f_3)$ updates both state and the set of formulas associated to each node as follows.
%
Although $\init^{\varphi}_{\mathcal{L}}$ and $\eta_1$ remain intact, but node $\eta_2$ is updated to $((d_1, d_2, f_3),(0,1), \setof{ F })$ because
%
$\updfct_\varphi(\textbf{X}_\beta d_3 \wedge \varphi,f_3)=F$. 
%
Moreover, node $\eta_3$ is updated to $\eta_3 = ((\bot, \bot, f_3),(1,1), \setof{ F , ( \textbf{X}_\beta f_1)\wedge \varphi, ( \textbf{X}_\beta f_1)\wedge \varphi})$.
%

The update event $(\beta_2,f_2)$  updates nodes $\eta_1$ and $\eta_3$ such that $\eta_1 = ((\bot, f_2, d_3), (1,0), \{\varphi \})$ and 
$\eta_3 = ((\bot, f_2, f_3),$ $(1,1),\setof{ F , ( \textbf{X}_\beta f_1)\wedge \varphi , ( \textbf{X}_\beta f_1)\wedge \varphi})$.
%

By observing the action event $(\drain_{23},(1,2))$, the new node $\eta_4 = ((\bot, \bot, \bot),(1,2), \{F ,(\textbf{X}_\beta d_3 \vee \textbf{X}_\beta f_1) \wedge ( \textbf{X}_\beta f_1)\wedge \varphi,(\textbf{X}_\beta d_3 \vee \textbf{X}_\beta f_1) \wedge ( \textbf{X}_\beta f_1)\wedge \varphi\})$ is created.
%

The update event $(\beta_1,f_1)$ updates nodes $\eta_1$, $\eta_3$ and $\eta_4$ such that $\eta_1 = ((f_1, f_2, d_3),(1,0), \setof{\varphi })$,  $\eta_3 = ((f_1, f_2, f_3),$ $(1,1), \setof{ F ,  \varphi,  \varphi})$ and $\eta_4 = ((f_1, \bot, \bot),(1,2), \setof{F ,  \varphi,  \varphi})$.
\end{example}
%   
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness of Formula Progression on the Lattice}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In \secref{sec:lattice}, we introduced how from an unobservable global trace $t$ of a distributed CBS with multi-party interactions one can construct a set of paths compatible with $t$ in form of a lattice.
%
Furthermore, in \secref{sec:ltl} we adapted formula progression over the constructed lattice with respect to a given LTL formula $\varphi$.
%
What we obtained is a directed lattice $\mathcal{L}^\varphi$ starting from the initial node and ending up with frontier node $\eta^f$.
%
The set of formulas attached to the frontier node, that is $\eta^f.\Sigma$, represents the progression of the initial formula over the set of path of the lattice.   
%
%
\begin{definition}[Progression on a global trace]
\label{def:bigprog}
Function $\PROG :  \LTL \times Q \cdot (\GActions \cdot Q)^*  \rightarrow \LTL $  is defined as:
%
\begin{itemize}
	\item
	$\PROG(\varphi, \init) = \varphi$,
	\item
	$\PROG(\varphi, \sigma)= \varphi'$
	\item
	$\PROG\left(\varphi, \sigma \cdot \left(\alpha \cup \beta\right)\cdot q\right)= \prog \left( \UPD \left(\PROG \left( \varphi , \sigma \right), \mathcal{Q} \right), q \right)$ where
	\begin{itemize}
		\item $\mathcal{Q} = \setof{q[i] \mid \beta_i \in \beta}$ is the set of updated states,
		\item function $\UPD: \LTL \times Q^R   \rightarrow \LTL$  is defined as:  
		\begin{itemize}
			\item $ \UPD \left( \varphi, \setof{\epsilon} \right)= \varphi$,
			\item $ \UPD \left( \varphi, Q^r \cup \setof{q_i} \right) = \updfct_\varphi \left(\UPD \left( \varphi, Q^r \right),q_i \right)$.
		\end{itemize}
	with $Q^R \subseteq \setof{ q \in Q^{\rm r}_i \lmid i \in [1,n]}$ the set of subsets of ready states of the components.
	\end{itemize}	
\end{itemize}
%
\end{definition}
%
Function $\PROG$ uses functions $\prog$, $\updfct_\varphi$ (Definitions~\ref{def:progression} and \ref{def:update}) and function $\UPD$.
%
Since after each global action we only have one global state (likely incomplete), function $\updfct_\varphi$ does not need to check among multiple global states to find whose formula must be updated. 
%
That is why $\PROG$ uses the simplified version of function $\updfct_\varphi$ by eliminating the scheduler index input. 
%
Moreover functions $\prog$ modified in such way to take as input a global state in $Q$ instead of a global state in $Q^l$ because as we above mentioned, the index of schedulers does not play a role in the progression of an LTL formula on a global trace. 
%

Given a global state $t$ as per \defref{def:global-trace} and an LTL property $\varphi$, by $\eta^f.\Sigma$ we denote the set of LTL formulas of the frontier node of the constructed computation lattice $\mathcal{L}^\varphi$, we have the two following proposition and theorems:
%
\begin{proposition}
\label{proposition:prog}
Given an LTL formula $\varphi$ and a global trace $t$, there exists a global trace $t'$ such that $\PROG(\varphi, t') =\mathit{progression} (\varphi, \mathcal{R}_\beta(t'))$ with:

\[
t' = \begin{dcases}
    t  &\text{ if } \last(t)[i] \in Q_i^{\rm r} \text{ for all } i \in [1\upto |\setofcomponents|], \\
   t \cdot \beta \cdot q  &\text{ otherwise.}
   \end{dcases}
\]
%
Where $ \beta \subseteq \bigcup_{i \in [1\upto |\setofcomponents|]} \setof{ \beta_i }$, $\forall i \in [1\upto |\setofcomponents|], q[i] \in Q_i^{\rm r}$ and $\mathit{progression}$ is the standard progression function described in~\cite{bauer12}.
\end{proposition}
%
Proposition~\ref{proposition:prog} states that progression of an LTL formula on a global trace of a distributed system, defined in \defref{def:global-trace}, using $\PROG$ is similar to the standard progression of the LTL formula on the corresponding refined global trace using $\mathit{progression}$.
%
Intuitively, progression of stabilized global trace $t$, results similar to the standard progression of refined $t$.
%
\begin{theorem}[Soundness]
\label{theorem:soundness}
For a global trace $t$ and LTL formula $\varphi$, we have   
\[
\forall \varphi' \in \eta^f.\Sigma , \exists t' \in \mathcal{P}(t) : \PROG(\varphi, t')= \varphi'.
\]
\end{theorem}
%
Theorem~\ref{theorem:soundness} states that each formula of the frontier node is derived from the progression of formula $\varphi$ on a compatible trace of trace $t$.
%
\begin{theorem}[Completeness]
\label{theorem:completeness}
For a global trace $t$ and an LTL formula $\varphi$, we have:
\[
\eta^f.\Sigma = \setof{\PROG(\varphi, t') \lmid t' \in \mathcal{P}(t) }.
\]
\end{theorem}
%
Theorem~\ref{theorem:completeness} states that the set of formulas in the frontier node is equal to the set of progression of $\varphi$ on all the compatible traces of $t$.
%

==> sharedcomponentevent.tex <==
\begin{algorithm}
\caption{\textsc{SharedComponentEvent}}
\begin{algorithmic}[1]
%
%
\Procedure{SharedComponentEvent}{$e$}
    \For {all $\eta \in \mathcal{L}.\mathit{nodes}$}	\label{line:start_update_nodes_shared}
			%\If {$\eta.\mathit{clock} \geq e.\mathit{clock}$}
			\If {$\eta.\mathit{clock} \geq \vc_{e.\mathit{sender}}^{e.\mathit{index}}$} \label{line:vc1}
			\Comment{nodes associated to executions that are happened after the last execution of scheduler $S_{e.\mathit{sender}}$ involving shared component $B_{e.\mathit{index}}$.}
				\State {$updatable \gets \true$}
					\For {all $j\in [1,m]\setminus \{e.\mathit{sender}\} \wedge e.\mathit{index} \in \scope(j)$}
							\If {$\eta.\mathit{clock} \geq  \vc_j^{e.\mathit{index}}$} \label{line:vc2}
							\Comment{nodes associated to executions that are happened after the last execution of  schedulers but $S_{e.\mathit{sender}}$ involving shared component $B_{e.\mathit{index}}$.}
								\State {$updatable \gets \false$}
								\State {\textbf{break}}
							\EndIf
					\EndFor
			\EndIf
			\If {$updatable$}
				\State {$\eta \gets \updb(\eta,e)$} \label{line:updatable}
			\EndIf
		\EndFor \label{line:end_update_nodes_shared}
\EndProcedure
%
\end{algorithmic}
\end{algorithm}

==> updatev.tex <==
\begin{algorithm}
\caption{\textsc{UpdateV}}
\label{alg:updatev}
\begin{algorithmic}[1]
%
%
\Procedure{UpdateV}{$e$}
	\State{$j \gets \managed(e).\mathit{index}$} \label{line:start_last_vc}
	\For {all $i \in \{i \in [1,n] \mid  B_i\in B_{\rm {s}} \wedge i \in \scope(j) \wedge i \in \involved(e.\mathit{action})\}$}	
		\State {$\vc_j^i \gets e.\mathit{clock}$}
		\Comment{store the vector clock in the dedicated variable.}
		\label{line:last_vc}
	\EndFor \label{line:end_last_vc}
\EndProcedure
%
\end{algorithmic}
%
\end{algorithm}
